A Bayesian partial identification approach to inferring the prevalence of accounting misconduct

This paper describes the use of flexible Bayesian regression models for estimating a partially identified probability function. Our approach permits efficient sensitivity analysis concerning the posterior impact of priors on the partially identified component of the regression model. The new methodology is illustrated on an important problem where only partially observed data is available - inferring the prevalence of accounting misconduct among publicly traded U.S. businesses.

==> BART_lit_review.tex <==
% \documentclass[11pt]{article}
% \usepackage[left=1in,top=1in,right=1in,bottom=1in]{geometry}
% \usepackage{amsmath}
% \usepackage{amsbsy}
% \usepackage{hyperref}
% \usepackage{graphicx,amsmath,amssymb,fullpage,amsfonts,bbm,bbold}
% \usepackage{fancyhdr}
% \usepackage{bbm}

% \usepackage{amsthm}
% \usepackage{epsfig}
% \usepackage{color}
% \usepackage{setspace}

% \linespread{2} 

% \newcommand{\logit}{\mbox{logit}}
% \newcommand{\B}{\mathbf{B}}
% \newcommand{\bPsi}{\mathbf{\Psi}}
% \newcommand{\bbeta}{\boldsymbol{\beta}}
% \newcommand{\bLambda}{\boldsymbol{\Lambda}}

% \newcommand{\X}{\mathbf{X}}
% \newcommand{\Z}{\mathbf{Z}}
% \newcommand{\br}{\mathbf{r}}
% \newcommand{\bv}{\mathbf{b}}
% \newcommand{\f}{\mathbf{f}}
% \newcommand{\btheta}{\boldsymbol{\theta}}

% \newcommand{\F}{\mathbf{F}}
% \newcommand{\z}{\mathbf{z}}
% \newcommand{\bSigma}{\boldsymbol{\Sigma}}

% \newcommand{\probit}{\mbox{probit}}
% \newcommand{\hiw}{\mbox{{\small\textsc{HIW}}}}
% \newcommand{\iw}{\mbox{{\small\textsc{IW}}}}
% \newcommand{\N}{\mbox{{\small\textsc{N}}}}
% \newcommand{\T}{\mbox{{\small\textsc{T}}}}
% \newcommand{\C}{\mbox{{\small\textsc{C}}}}
% \newcommand{\Ga}{\mbox{{\small\textsc{Ga}}}}
% \newcommand{\IG}{\mbox{{\small\textsc{IG}}}}
% \newcommand{\Be}{\mbox{{\small\textsc{Be}}}}
% \newcommand{\Ber}{\mbox{{\small\textsc{Ber}}}}
% \newcommand{\dd}{\mbox{d}}
% \newcommand{\E}{\mbox{E}}
% \newcommand{\V}{\mathbf{V}}
% \newcommand{\I}{\mathbf{I}}
% \newcommand{\Tau}{\mathrm{T}}
% \newcommand{\sayan}[1] {{\textcolor{red}{ #1}}}
% \newtheorem{theorem}{Theorem}[section]
% \DeclareMathOperator{\iid}{\stackrel{\mbox{\tiny iid} }{\sim}}

% \newenvironment{example}[1][Example]{\begin{trivlist}
% \item[\hskip \labelsep {\bfseries #1}]}{\end{trivlist}}
% \newenvironment{remark}[1][Remark]{\begin{trivlist}
% \item[\hskip \labelsep {\bfseries #1}]}{\end{trivlist}}
% \usepackage{bm}
% \usepackage{natbib}


% \begin{document}


%Binary regression of a response variable $Y$ on predictors $X$ aims to model
%$$P(Y_i=1\mid x_i)=f(x_i),$$ where the functional form of $f(\cdot)$ depends on assumptions about the relationship of outcome and predictors. 

%Parametric modelling of binary regression has been extensively studied in the literature, the most common approaches being logistic and probit regression  \citep{cox1958regression}. 
%Aside from computational gains and efficient inferences, logistic and probit regression both offer additional benefits since they retain identifiability even in pathological regimes of non-random sampling, as long as there is at least one exclusion restriction \cite{poirier1980partial}. 

%However, although both of these approaches are flexible, they assume restrictive forms for the shape of the response probabilities and can lead to biased inferences when the modelling assumptions are violated \cite{hastie2013inference}. Flexible non-parametric alternatives to binary regression have been introduced in the past few years, allowing relaxation of parametric assumptions. Examples of such methods include Bayesian non-parametric modelling of both outcomes and predictors \cite{dunson2008bayesian} and profile regression \cite{molitor2010bayesian}. These methods assume an underlying base distribution for mixture components within a non-parametric framework, using the smoothness of the base distribution in order to borrow information across observations. 

%A popular alternative to assuming smoothness of $f(\cdot)$ is to employ regression trees, which were first introduced in classification and prediction contexts (see \cite{breiman2001random,evers2009locally}). 


In our application, the nonlinear function $\theta(\X)$ was modeled using the Bayesian Additive Regression Trees (BART) approach of \cite{chipman2010bart}. BART is more flexible than classical parametric regression models, such as linear logistic or probit regression \citep{cox1958regression}. Relative to competing nonparametric Bayesian regression models, BART is particularly well-suited to detecting interactions and discontinuities, and it is invariant to monotone transformations of the covariates. For clarity, in this appendix we keep to the original notation used in \cite{chipman2010bart}; several of the BART prior parameter names are used in the main text but refer to different entities.

 % and does not rely on smoothness assumptions as do popular modern alternatives \citep{molitor2010bayesian, dunson2008bayesian}.

The BART prior represents an unknown function $f(\X)$ as a sum of many piecewise constant binary regression trees.
%Each of the trees in BART can pick up `weak' patterns in the data, such that the sum of all trees provides a combined representation of many such signals. The particular appeal in our context is its ability to detect inohmogeneous  response surfaces including discontinuities \cite{hill2011bayesian} and to pick up interactions in the predictors, as well as its computational efficiency. 
%$\mathcal{T}=\left\{T_1,\ldots,T_L\right\}$. 
%, building off earlier tree-based regression models \citep{breiman2001random,evers2009locally}. 
%
Each tree $T_l,\;1\leq l\leq L$, consists of a set of internal decision nodes which define a partition of the covariate space (say $\mathcal{A}_1,\dots,\mathcal{A}_{B(l)}$), as well as a set of terminal nodes or leaves --- one corresponding to each element of the partition. Each subset of the partition $\mathcal{A}_b$ is associated with a parameter value $\mu_{lb}$, defining a piecewise constant function: $g_l(x) = \mu_{lb}\ \text{if}\ x\in \mathcal{A}_b.$ This regression tree function representation is depicted in Figure \ref{trepan}. 
%, so as to describe a function $g_l(x)$ which is piecewise constant.  In other words, each tree defines a decision rule of the form $\left\{\X\in A\right\}$ vs  $\left\{\X\not\in A\right\}$, partitioning the covariate space into disjoint regions. Conditional on this partition, a constant mean function is fit to the data in each disjoint region. 

\include{fig/fig.tex}

Individual regression trees are then additively combined into a single regression function: $f(\X)=\sum_{l=1}^L g_l(\X).$ The representation of $f(\X)$ through the sum of a set of regression trees is generally non-unique; in our applications, this redundancy is unproblematic.

Each of the functions $g_l$ are constrained by their prior to be ``weak learners"; that is, the prior strongly favors small trees and leaf parameters that are near zero. Each tree independently follows the prior described by \cite{chipman1998bayesian}, where the probability that a node at depth $d$ splits (is not terminal) is given by 
$\alpha (1+d)^{-\beta},\;\;\alpha\in (0,1),\;\beta\in [0,\infty).$

A variable to split on, and a cut-point to split at, are then selected uniformly at random from the available splitting rules.  Large, deep trees are given extremely low prior probability by taking $\alpha=0.95$ and $\beta=2$ as in \cite{chipman2010bart}. 
The leaf parameters are assigned independent priors
$\mu_{lb}\sim N(0,\sigma^2_\mu)\;\;\textrm{ where }\sigma_\mu=3/(k\sqrt{L})$. The default  value, $k=2$, shrinks $g_l(x)$ strongly toward zero. The induced prior for $f(x)$ is centered at zero and puts approximately 95\% of the prior mass within $\pm 3$ pointwise. Larger values of $k$ imply increasing degrees of shrinkage.

Finally, the probability function of interest is modeled as $\Phi\left(f(\X)+c\right)$, where $c$ is an offset. Complete details of the BART prior and its implementation are given by \cite{chipman2010bart}.



%This shrinks $f(\X)$ towards . so that the probability $\mbox{Pr}(Y=1\mid \X)=\Phi\left(f(\X)+c\right)$ is ``shrunk" towards $\Phi\left(c\right)$. A high or low value of $c$ represents an a priori expectation of high or low prevalence respectively. 
%

%Its flexibility allows it to detect inhomogeneous response surfaces including discontinuities \cite{hill2011bayesian}.
% BART is able to detect interactions and nonlinearities in the response surface, which (among other advantages) allows it to more readily identify heterogeneous treatment effects.

 % \cite{hill2011bayesian}

%COPY-PASTE FROM BART PAPER:\\
%To do this, we consider modeling or at least approximating f (x) = E􏱇(Y |x), the mean of Y given x, by a sum of m regression trees f(x) = h(x)	mj=1 gj(x) where each gj denotes a regression tree. Thus, we approximate (1) by a sum-of- trees model. A sum-of-trees model is fundamentally an additive model with multivariate components. Compared to generalized additive models based on sums of low di-mensional smoothers, these multivariate components can more naturally incorpo- rate interaction effects. And compared to a single tree model, the sum-of-trees can more easily incorporate additive effects. Various methods which combine a set of tree models, so called ensemble methods, have attracted much attention. These include boosting [Freund and Schapire (1997), Friedman (2001)], bagging [Breiman (1996)] and random forests [Breiman (2001)], each of which use different techniques to fit a linear combination of trees.
% Boosting fits a sequence of single trees, using each tree to fit data variation not explained by earlier trees in the sequence. Bagging and random forests use randomization to create a large number of independent trees, and then reduce prediction variance by averaging predictions across the trees.

% Yet another approach that results in a linear combination of trees is Bayesian model averaging applied to the posterior arising from a Bayesian single-tree model as in Chipman, George and McCulloch (1998) (hereafter CGM98), Denison, Mallick and Smith (1998), Blanchard (2004) and Wu, Tjelmeland and West (2007). Such model averaging uses posterior probabilities as weights for averaging the predictions from individual trees.

%In this paper we propose a Bayesian approach called BART (Bayesian Additive Regression Trees) which uses a sum of trees to model or approximate f (x) = E(Y|x). The essential idea is to elaborate the sum-of-trees model (2) by imposing a prior that regularizes the fit by keeping the individual tree effects small. In effect, the gj ’s become a dimensionally adaptive random basis of ``weak learners,'' to borrow a phrase from the boosting literature. By weakening the gj effects, BART ends up with a sum of trees, each of which explains a small and different portion of f . Note that BART is not equivalent to posterior averaging of single tree fits of the entire function f .

%COPY-PASTE FROM HILL PAPER: \\
%Given recent advances in Bayesian nonparametric models with extremely flexible func- tional form, this article proposes that a robust, yet simpler, modeling approach is now available for accurately estimating causal effects in this setting. This approach focuses on precise modeling of the response surface using a nonparametric (or, equivalently, very highly parametric) modeling strategy called Bayesian Additive Regression Trees, or BART (Chipman, George, and McCulloch 2007, 2010). The BART algorithm is straightforward to implement and requires the researcher only to input the outcome, treatment assignment, and confounding covariates, but requires no information about how these variables are parametrically related. Yet BART is able to detect interactions and nonlinearities in the response surface, which (among other advan- tages) allows it to more readily identify heterogeneous treatment effects. Also, BART natu- rally produces coherent posterior intervals in contrast to methods such as propensity score matching and subclassification, for instance, for which there is still no consensus regarding appropriate interval estimation (Imbens 2004; Hill and Reiter 2006) (though Abadie and Imbens 2006 recently proposed an estimator that may be a viable solution under certain conditions). Finally, treatment effect point estimates calculated using BART appear to be substantially more accurate (for instance, as measured by root mean squared error) in the nonlinear settings considered here than estimates from equally accessible competitors such as linear regression, propensity-weighted estimators, and propensity score matching with regression adjustment. Even when the response surface is linear with additive treatment effects, BART’s performance in simulations is almost indistinguishable from linear regres- sion, the “correct” model for that setting. Thus BART is a simple method that appears to have the potential to be both robust and accurate in the estimation of causal effects.

%\bibliographystyle{plainnat}
%\bibliography{bib/biased_sampling_bart}
%\end{document}  

==> JASA_revised copy/BART_lit_review.tex <==
% \documentclass[11pt]{article}
% \usepackage[left=1in,top=1in,right=1in,bottom=1in]{geometry}
% \usepackage{amsmath}
% \usepackage{amsbsy}
% \usepackage{hyperref}
% \usepackage{graphicx,amsmath,amssymb,fullpage,amsfonts,bbm,bbold}
% \usepackage{fancyhdr}
% \usepackage{bbm}

% \usepackage{amsthm}
% \usepackage{epsfig}
% \usepackage{color}
% \usepackage{setspace}

% \linespread{2} 

% \newcommand{\logit}{\mbox{logit}}
% \newcommand{\B}{\mathbf{B}}
% \newcommand{\bPsi}{\mathbf{\Psi}}
% \newcommand{\bbeta}{\boldsymbol{\beta}}
% \newcommand{\bLambda}{\boldsymbol{\Lambda}}

% \newcommand{\X}{\mathbf{X}}
% \newcommand{\Z}{\mathbf{Z}}
% \newcommand{\br}{\mathbf{r}}
% \newcommand{\bv}{\mathbf{b}}
% \newcommand{\f}{\mathbf{f}}
% \newcommand{\btheta}{\boldsymbol{\theta}}

% \newcommand{\F}{\mathbf{F}}
% \newcommand{\z}{\mathbf{z}}
% \newcommand{\bSigma}{\boldsymbol{\Sigma}}

% \newcommand{\probit}{\mbox{probit}}
% \newcommand{\hiw}{\mbox{{\small\textsc{HIW}}}}
% \newcommand{\iw}{\mbox{{\small\textsc{IW}}}}
% \newcommand{\N}{\mbox{{\small\textsc{N}}}}
% \newcommand{\T}{\mbox{{\small\textsc{T}}}}
% \newcommand{\C}{\mbox{{\small\textsc{C}}}}
% \newcommand{\Ga}{\mbox{{\small\textsc{Ga}}}}
% \newcommand{\IG}{\mbox{{\small\textsc{IG}}}}
% \newcommand{\Be}{\mbox{{\small\textsc{Be}}}}
% \newcommand{\Ber}{\mbox{{\small\textsc{Ber}}}}
% \newcommand{\dd}{\mbox{d}}
% \newcommand{\E}{\mbox{E}}
% \newcommand{\V}{\mathbf{V}}
% \newcommand{\I}{\mathbf{I}}
% \newcommand{\Tau}{\mathrm{T}}
% \newcommand{\sayan}[1] {{\textcolor{red}{ #1}}}
% \newtheorem{theorem}{Theorem}[section]
% \DeclareMathOperator{\iid}{\stackrel{\mbox{\tiny iid} }{\sim}}

% \newenvironment{example}[1][Example]{\begin{trivlist}
% \item[\hskip \labelsep {\bfseries #1}]}{\end{trivlist}}
% \newenvironment{remark}[1][Remark]{\begin{trivlist}
% \item[\hskip \labelsep {\bfseries #1}]}{\end{trivlist}}
% \usepackage{bm}
% \usepackage{natbib}


% \begin{document}


%Binary regression of a response variable $Y$ on predictors $X$ aims to model
%$$P(Y_i=1\mid x_i)=f(x_i),$$ where the functional form of $f(\cdot)$ depends on assumptions about the relationship of outcome and predictors. 

%Parametric modelling of binary regression has been extensively studied in the literature, the most common approaches being logistic and probit regression  \citep{cox1958regression}. 
%Aside from computational gains and efficient inferences, logistic and probit regression both offer additional benefits since they retain identifiability even in pathological regimes of non-random sampling, as long as there is at least one exclusion restriction \cite{poirier1980partial}. 

%However, although both of these approaches are flexible, they assume restrictive forms for the shape of the response probabilities and can lead to biased inferences when the modelling assumptions are violated \cite{hastie2013inference}. Flexible non-parametric alternatives to binary regression have been introduced in the past few years, allowing relaxation of parametric assumptions. Examples of such methods include Bayesian non-parametric modelling of both outcomes and predictors \cite{dunson2008bayesian} and profile regression \cite{molitor2010bayesian}. These methods assume an underlying base distribution for mixture components within a non-parametric framework, using the smoothness of the base distribution in order to borrow information across observations. 

%A popular alternative to assuming smoothness of $f(\cdot)$ is to employ regression trees, which were first introduced in classification and prediction contexts (see \cite{breiman2001random,evers2009locally}). 


In our application, the nonlinear function $\theta(\X)$ was modeled using the Bayesian Additive Regression Trees (BART) approach of \cite{chipman2010bart}. BART is more flexible than classical parametric regression models, such as linear logistic or probit regression \citep{cox1958regression}. Relative to competing nonparametric Bayesian regression models, BART is particularly well-suited to detecting interactions and discontinuities, and it is invariant to monotone transformations of the covariates. For clarity, in this appendix we keep to the original notation used in \cite{chipman2010bart}; several of the BART prior parameter names are used in the main text but refer to different entities.

 % and does not rely on smoothness assumptions as do popular modern alternatives \citep{molitor2010bayesian, dunson2008bayesian}.

The BART prior represents an unknown function $f(\X)$ as a sum of many piecewise constant binary regression trees.
%Each of the trees in BART can pick up `weak' patterns in the data, such that the sum of all trees provides a combined representation of many such signals. The particular appeal in our context is its ability to detect inohmogeneous  response surfaces including discontinuities \cite{hill2011bayesian} and to pick up interactions in the predictors, as well as its computational efficiency. 
%$\mathcal{T}=\left\{T_1,\ldots,T_L\right\}$. 
%, building off earlier tree-based regression models \citep{breiman2001random,evers2009locally}. 
%
Each tree $T_l,\;1\leq l\leq L$, consists of a set of internal decision nodes which define a partition of the covariate space (say $\mathcal{A}_1,\dots,\mathcal{A}_{B(l)}$), as well as a set of terminal nodes or leaves --- one corresponding to each element of the partition. Each subset of the partition $\mathcal{A}_b$ is associated with a parameter value $\mu_{lb}$, defining a piecewise constant function: $g_l(x) = \mu_{lb}\ \text{if}\ x\in \mathcal{A}_b.$ This regression tree function representation is depicted in Figure \ref{trepan}. 
%, so as to describe a function $g_l(x)$ which is piecewise constant.  In other words, each tree defines a decision rule of the form $\left\{\X\in A\right\}$ vs  $\left\{\X\not\in A\right\}$, partitioning the covariate space into disjoint regions. Conditional on this partition, a constant mean function is fit to the data in each disjoint region. 

\include{fig/fig.tex}

Individual regression trees are then additively combined into a single regression function: $f(\X)=\sum_{l=1}^L g_l(\X).$ The representation of $f(\X)$ through the sum of a set of regression trees is generally non-unique; in our applications, this redundancy is unproblematic.

Each of the functions $g_l$ are constrained by their prior to be ``weak learners"; that is, the prior strongly favors small trees and leaf parameters that are near zero. Each tree independently follows the prior described by \cite{chipman1998bayesian}, where the probability that a node at depth $d$ splits (is not terminal) is given by 
$\alpha (1+d)^{-\beta},\;\;\alpha\in (0,1),\;\beta\in [0,\infty).$

A variable to split on, and a cut-point to split at, are then selected uniformly at random from the available splitting rules.  Large, deep trees are given extremely low prior probability by taking $\alpha=0.95$ and $\beta=2$ as in \cite{chipman2010bart}. 
The leaf parameters are assigned independent priors
$\mu_{lb}\sim N(0,\sigma^2_\mu)\;\;\textrm{ where }\sigma_\mu=3/(k\sqrt{L})$. The default  value, $k=2$, shrinks $g_l(x)$ strongly toward zero. The induced prior for $f(x)$ is centered at zero and puts approximately 95\% of the prior mass within $\pm 3$ pointwise. Larger values of $k$ imply increasing degrees of shrinkage.

Finally, the probability function of interest is modeled as $\Phi\left(f(\X)+c\right)$, where $c$ is an offset. Complete details of the BART prior and its implementation are given by \cite{chipman2010bart}.



%This shrinks $f(\X)$ towards . so that the probability $\mbox{Pr}(Y=1\mid \X)=\Phi\left(f(\X)+c\right)$ is ``shrunk" towards $\Phi\left(c\right)$. A high or low value of $c$ represents an a priori expectation of high or low prevalence respectively. 
%

%Its flexibility allows it to detect inhomogeneous response surfaces including discontinuities \cite{hill2011bayesian}.
% BART is able to detect interactions and nonlinearities in the response surface, which (among other advantages) allows it to more readily identify heterogeneous treatment effects.

 % \cite{hill2011bayesian}

%COPY-PASTE FROM BART PAPER:\\
%To do this, we consider modeling or at least approximating f (x) = E􏱇(Y |x), the mean of Y given x, by a sum of m regression trees f(x) = h(x)	mj=1 gj(x) where each gj denotes a regression tree. Thus, we approximate (1) by a sum-of- trees model. A sum-of-trees model is fundamentally an additive model with multivariate components. Compared to generalized additive models based on sums of low di-mensional smoothers, these multivariate components can more naturally incorpo- rate interaction effects. And compared to a single tree model, the sum-of-trees can more easily incorporate additive effects. Various methods which combine a set of tree models, so called ensemble methods, have attracted much attention. These include boosting [Freund and Schapire (1997), Friedman (2001)], bagging [Breiman (1996)] and random forests [Breiman (2001)], each of which use different techniques to fit a linear combination of trees.
% Boosting fits a sequence of single trees, using each tree to fit data variation not explained by earlier trees in the sequence. Bagging and random forests use randomization to create a large number of independent trees, and then reduce prediction variance by averaging predictions across the trees.

% Yet another approach that results in a linear combination of trees is Bayesian model averaging applied to the posterior arising from a Bayesian single-tree model as in Chipman, George and McCulloch (1998) (hereafter CGM98), Denison, Mallick and Smith (1998), Blanchard (2004) and Wu, Tjelmeland and West (2007). Such model averaging uses posterior probabilities as weights for averaging the predictions from individual trees.

%In this paper we propose a Bayesian approach called BART (Bayesian Additive Regression Trees) which uses a sum of trees to model or approximate f (x) = E(Y|x). The essential idea is to elaborate the sum-of-trees model (2) by imposing a prior that regularizes the fit by keeping the individual tree effects small. In effect, the gj ’s become a dimensionally adaptive random basis of ``weak learners,'' to borrow a phrase from the boosting literature. By weakening the gj effects, BART ends up with a sum of trees, each of which explains a small and different portion of f . Note that BART is not equivalent to posterior averaging of single tree fits of the entire function f .

%COPY-PASTE FROM HILL PAPER: \\
%Given recent advances in Bayesian nonparametric models with extremely flexible func- tional form, this article proposes that a robust, yet simpler, modeling approach is now available for accurately estimating causal effects in this setting. This approach focuses on precise modeling of the response surface using a nonparametric (or, equivalently, very highly parametric) modeling strategy called Bayesian Additive Regression Trees, or BART (Chipman, George, and McCulloch 2007, 2010). The BART algorithm is straightforward to implement and requires the researcher only to input the outcome, treatment assignment, and confounding covariates, but requires no information about how these variables are parametrically related. Yet BART is able to detect interactions and nonlinearities in the response surface, which (among other advan- tages) allows it to more readily identify heterogeneous treatment effects. Also, BART natu- rally produces coherent posterior intervals in contrast to methods such as propensity score matching and subclassification, for instance, for which there is still no consensus regarding appropriate interval estimation (Imbens 2004; Hill and Reiter 2006) (though Abadie and Imbens 2006 recently proposed an estimator that may be a viable solution under certain conditions). Finally, treatment effect point estimates calculated using BART appear to be substantially more accurate (for instance, as measured by root mean squared error) in the nonlinear settings considered here than estimates from equally accessible competitors such as linear regression, propensity-weighted estimators, and propensity score matching with regression adjustment. Even when the response surface is linear with additive treatment effects, BART’s performance in simulations is almost indistinguishable from linear regres- sion, the “correct” model for that setting. Thus BART is a simple method that appears to have the potential to be both robust and accurate in the estimation of causal effects.

%\bibliographystyle{plainnat}
%\bibliography{bib/biased_sampling_bart}
%\end{document}  

==> JASA_revised copy/fig/fig.tex <==



\begin{figure}
\begin{center}
\begin{tikzpicture}[
  scale=1.1,
    node/.style={%
      draw,
      rectangle,
    },
    node2/.style={%
      draw,
      circle,
    },
  ]

    \node [node] (A) {$x_1<0.8$};
    \path (A) ++(-135:\nodeDist) node [node2] (B) {$\mu_{h1}$};
    \path (A) ++(-45:\nodeDist) node [node] (C) {$x_2<0.4$};
    \path (C) ++(-135:\nodeDist) node [node2] (D) {$\mu_{h2}$};
    \path (C) ++(-45:\nodeDist) node [node2] (E) {$\mu_{h3}$};

    \draw (A) -- (B) node [left,pos=0.25] {no}(A);
    \draw (A) -- (C) node [right,pos=0.25] {yes}(A);
    \draw (C) -- (D) node [left,pos=0.25] {no}(A);
    \draw (C) -- (E) node [right,pos=0.25] {yes}(A);
\end{tikzpicture}
%
\hspace{0.1\linewidth}
\begin{tikzpicture}[scale=4]
\draw [thick, -] (0,1) -- (0,0) -- (1,0) -- (1,1)--(0,1);
\draw [thin, -] (0.8, 1) -- (0.8, 0);
\draw [thin, -] (0.0, 0.4) -- (0.8, 0.4);
\node at (-0.1,0.4) {0.4};
\node at (0.8,-0.1) {0.8};
\node at (0.5,-0.2) {$x_1$};
\node at (-0.3,0.5) {$x_2$};
\node at (0.9,0.5) {$\mu_{h1}$};
\node at (0.4,0.7) {$\mu_{h2}$};
\node at (0.4,0.2) {$\mu_{h3}$};
\end{tikzpicture}
\end{center}
\caption{(Left) An example binary tree, with internal nodes labelled by their splitting rules and terminal nodes labelled with the corresponding parameters $\mu_{hb}$ (Right) The corresponding partition of the sample space and the step function.}
\label{fig:treestep}
\end{figure}



==> JASA_revised copy/flu.tex <==
%!TEX root = HahnMurrayManolopoulouSupplement.tex

Our data come from a randomized encouragement study of the effectiveness of an influenza vaccine conducted at an academic primary care practice affiliated with a large teaching hospital in an urban setting \citep{McDonald1992}. Physicians were randomly assigned to treatment or control groups, with treated physicians receiving a computerized reminder about the vaccine when a patient with a scheduled visit also met the U.S. Public Health Service Criteria for receiving a flu vaccine. Patients were eligible for the vaccine if they were 65 or older, or if they had certain severe chronic diseases including chronic obstructive pulmonary disease (COPD).
% lung disease, asthma, diabetes, congestive heart failure, or severe liver or kidney failure. 
The outcome of interest is subsequent hospitalization for flu-related illness, and the covariates include the patient's age and COPD status. \cite{Hirano2000} conduct a Bayesian analysis of this problem, placing a default joint prior over all the identified and unidentified parameters. In this application we perform an alternative selectively informative analysis with modular priors. %One aspect of this design which has been ignored to date is that the inclusion criteria potentially induce a sharp change in the probability of a positive outcome at age 65, since anyone 65 or older was in the study population while a 64 year-old patient would only be included if he or she had a serious, chronic disease.
We will use the terms ``reminder'', ``instrument'' and ``encouragement'' interchangably here, prefering ``reminder'' in the context of the specific applied problem.
 
\subsection{Causal Inference in a Binary Instrumental Variables Model}
%\sayan{fix to make everything conditional on X (doesn't change anything substantively)} 

Let $Z_i, T_i$, and $Y_i$ be the observed values of the treatment assignment (or encouragement, or instrument), treatment received, and outcome for observation $i$, respectively.  Let $X_i$ be a vector of baseline covariates. In the flu data, $Z_i=1$ if encouragement (the reminder) was administered, $T_i=1$ if the vaccine was administered, and $Y_i=1$ if the patient was \emph{not} hospitalized. As in \cite{Angrist1996} and \cite{Hirano2000} define the \emph{potential outcomes} $T_i(z)$ and $ Y_i(t,z)$ as the treatment
assignment that would have been observed had we fixed $Z_i=z$ and the outcome we would have observed fixing $T_i=t, Z_i=z$, respectively. We will suppress indexing by $i$ for population quantities. We make the stable unit treatment value assumption (SUTVA) \citep{Angrist1996}, i.e. that there is no interference between units and no alternative versions of treatment. \footnote{\cite{Hirano2000} point out that in an infectious disease application with individuals as the unit of randomization this assumption is unlikely to hold exactly, but constitutes a reasonable first order approximation.} Mathematically, SUTVA implies that $T_i(\mathbf{z})=T_i(z_i)$ and $Y_i(\mathbf{t}, \mathbf{z})=Y_i(t_i, z_i)$, where $\mathbf{z}, \mathbf{t}$ are vectors of instrument/encouragement assignment and treatments received (respectively) for the entire sample.

In this application the complete vector of binary response variables is 
\begin{equation}
U_i=(T_i(0), T_i(1), Y_i(0,0), Y_i(0,1), Y_i(1,0), Y_i(1,1))',
\end{equation}
 the collection of treatments and outcomes under all possible experimental conditions. However, we observe only $T_i\equiv T_i(Z_i)$ and $Y_i\equiv Y_i(T_i(Z_i), Z_i)$, where $Z_i$ is randomly assigned at the study outset. 
%
%as follows:
%\begin{equation}
%T_i = Z_iT_i(1) + (1-Z_i)T_i(0)
%\end{equation}
%\begin{equation}
% Y_i = T_iZ_iY_i(1,1) + 
%(1-T_i)Z_iY_i(0,1) + 
%T_i(1-Z_i)Y_i(1,0) + 
%(1-T_i)(1-Z_i)Y_i(0,0).
%\end{equation}
%
We can define compliance types or principal strata $S$ based on the possible values for $(T(1), T(0))$ -- see Table \ref{tab:comptype}. 
%
\begin{table}
\begin{center}
    \begin{tabular}{cc|ll}
        $T(1)$ & $T(0)$ & $S$ (Compliance Type) & ~    \\ \hline
        0     & 0     & Never Taker     & (n) \\ 
        1     & 1     & Always Taker    & (a) \\ 
        1     & 0     & Complier        & (c) \\ 
        0     & 1     & Defier          & (d) \\
    \end{tabular}
  \caption{Compliance types, or principal strata, defined by response patterns across levels of $Z$.}
  \label{tab:comptype}
  \end{center}
\end{table}
%
We will assume that the encouragement $Z$ is ignorable or randomly assigned (as it is in the flu data).
We also assume that there are no defiers (``monotonicity of compliance"), i.e., $ \Pr(S=d\mid \X)=0$. In the current setting a defier would be a patient who would \emph{only} receive the vaccine if the reminder was \emph{not} administered, which is quite unlikely.

Let $\pi_s(x) = \Pr(S=s\mid \X)$  and 
$\gamma^{tz}_s(x) = \Pr( Y(t,z)=1\mid S=s, \X)$ denote the principal strata and potential outcome probability models. Under the above assumptions the potential outcome and principal strata distributions are linked to the joint distribution of observables by the following equations.
%
\begin{align}
\Pr(T=1\mid Z=0, \X) &= \pi_a(\X)\label{eq:mon-1},\\
\Pr(T=1\mid Z=1, \X) &= \pi_c(\X) + \pi_a(\X)\label{eq:mon-2},\\
\Pr(Y=1\mid T=0, Z=0, \X) &= [\pi_c(\X)\gamma^{00}_c(\X) + \pi_n(\X)\gamma^{00}_n(\X)]/[\pi_c(\X) + \pi_n(\X)]\label{eq:mon-3},\\
\Pr(Y=1\mid T=1, Z=1, \X) &= [\pi_c(\X)\gamma^{11}_c(\X) + \pi_a(\X)\gamma^{11}_a(\X)]/[\pi_c(\X) + \pi_a(\X)]\label{eq:mon-4},\\
\Pr(Y=1\mid T=0, Z=1, \X) &= \gamma^{01}_n(\X),\\
\Pr(Y=1\mid T=1, Z=0, \X) &= \gamma^{10}_a(\X)\label{eq:mon-last}.
\end{align}
\cite{Richardson2010} derive this mixture relationship between principal strata/potential outcome distributions and the observable joint in detail under a range of assumptions about the latent variables (see also \cite{Imbens1997a} and \cite{Richardson2011}).

The probabilities on the left hand side completely determine the joint distribution of observables ($Y$ and $T$ given $Z$) and hence constitute a basis for $\phi$. Clearly $\pi$, $\gamma^{01}_n$ and $\gamma^{10}_a$ are one-to-one maps from $\phi$, and are point identified as well. However, $\gamma^{00}_c,\ \gamma^{00}_n,\ \gamma^{11}_c,$ and $ \gamma^{11}_a$ are not. For example, at any point in covariate space $\gamma^{11}_c(x)$ and $\gamma^{11}_a(x)$ must lie on the line segment given by the intersection of the line in equation \eqref{eq:mon-4} and $[0,1]\times [0,1]$, but the data are wholly uninformative about their position on that line segment. In particular, the range of $\gamma^{11}_a(x)$ is

\begin{equation}
\left(
	\min\left(
		0, \frac{\pi_a(x)+\pi_c(x)}{\pi_a(x)}p_{1\mid 11}(x) - \frac{\pi_c(x)}{\pi_a(x)}
	\right),\,
	\max\left(
		1, \frac{\pi_a(x)+\pi_c(x)}{\pi_a(x)}p_{1\mid 11}(x)
	\right)
\right)\label{eq:gbound}
\end{equation}
where $p_{1\mid 11}(x) = \Pr(Y=1\mid T=1, Z=1,\X)$. The situation is exactly the same for $\gamma^{00}_c(x)$ and $\gamma^{00}_n(x)$, with the line given by \eqref{eq:mon-3} and bounds similar to \eqref{eq:gbound} (large sample bounds on causal effects within principal strata were introduced by  \cite{zhang2003estimation}; see \cite{Richardson2011} for bounds under monotonicity and other assumptions, as well as further references).

%j 7/29
%In the instrumental variables literature, 
Point identification for the remaining parameters is often obtained through further assumptions on the distribution of the potential outcomes. The \emph{stochastic exclusion restriction} for compliance type $s$ posits that there is no direct effect of $Z$ on $Y$; that is, $\gamma^{i0}_s = \gamma^{i1}_s$ for $i=0,1$ \citep{Hirano2000}. From \eqref{eq:mon-1}-\eqref{eq:mon-last} it is clear that this achieves point identification for the entire distribution of the potential outcomes.

\cite{Hirano2000} anticipated failures of the exclusion restrictions, noting that a reminder about flu shots might also prompt physicians to counsel patients about other preventative measures to avoid contracting the flu. They propose relaxing the exclusion restrictions and resolving the resulting nonidentifiability through prior probability modeling. In this sense our approach and theirs are philosophically similar, but our framework affords us significant flexibility in choosing the model for $\phi$ while transparently embedding prior information about $\theta$, which is difficult to do in their modeling setup. In our subsequent analysis we will avoid imposing any exclusion restrictions.
%
% What will be particularly relevant for our  analysis is that any direct effect of the reminder on subsequent hospitalization for flu-related illness should be positive and relatively small, and is likely to be larger in always takers than in never takers (since one factor driving uptake of the vaccine and other prophylactic measures is perceived risk, which is higher in always takers).
%
%
%
%
%
%Our focus will be on \emph{intention-to-treat (ITT)} effects. The sample ITT effect is 
%
%\begin{equation}
%ITT = \frac{1}{n}\sum_{i=1}^n (Y_i(T_i(1), 1) - Y_i(T_i(0), 0)). 
%\end{equation}
%Sample ITT effects for different compliance types are defined similarly:
%\begin{equation}
%ITT_s = \frac{1}{n_s}\sum_{i: S_i=s} (Y_i(T_i(1), 1) - Y_i(T_i(0), 0)). 
%\end{equation}
%where $n_s$ is the number of observations with compliance type $S$ \citep{Hirano2000}. 
%The potential outcome distributions $\gamma$ and compliance type distributions $\pi$ are linked to the joint distribution of observables by the following equations (suppressing the dependence on $x$):
%
%\begin{align}
%\Pr(T=1\mid Z=0) &= \pi_D + \pi_a\\
%\Pr(T=1\mid Z=1) &= \pi_c + \pi_a\\
%\Pr(Y=1\mid T=0, Z=0) &= (\pi_c\gamma^{00}_c + \pi_n\gamma^{00}_n)/(\pi_c + \pi_n)\\
%\Pr(Y=1\mid T=1, Z=1) &= (\pi_c\gamma^{11}_c + \pi_a\gamma^{11}_a)/(\pi_c + \pi_a)\\
%\Pr(Y=1\mid T=0, Z=1) &= (\pi_D\gamma^{01}_D + \pi_n\gamma^{01}_n)/(\pi_D + \pi_n)\\
%\Pr(Y=1\mid T=1, Z=0) &= (\pi_D\gamma^{10}_D + \pi_a\gamma^{10}_a)/(\pi_D + \pi_a).
%\end{align}
%
% Assuming the exclusion restriction in always and never takers point identifies the (population) intent to treat effect in compliers:
%\begin{equation}
%PITT_{C} = \gamma^{11}_c - \gamma^{00}_c,
%\end{equation}
%which is equivalent to the local average treatment effect (LATE) if the exclusion restriction holds in compliers as well \cite{Angrist1996}. In the absence of the exclusion restrictions for always takers and/or compliers, $PITT_c$ is bounded by the equations above and the fact that the $\gamma$'s are probabilities. Since the data are informative about these bounds (the bounds themselves are point identified) $PITT_c$ is \emph{partially} identified.
%
%There are theoretical and empirical reasons to suspect that the exclusion restrictions might be violated. \cite{Richardson2011} give a detailed exposition of bounds on the joint distribution of $(Y, T\mid Z)$ induced by assuming various combinations of monotonicity and the exclusion restrictions.  \cite{Richardson2011} compute posterior distributions of these bounds under a Dirichlet-multinomial model without covariates. Assuming monotonicity, they find that the posterior probability of violating the bounds is 0.54 and 0.06 for the exclusion restriction in always takers and never takers respectively. Since the bounds are necessary but not sufficient for the exclusion restrictions to hold, there is ample evidence that the exclusion restrictions are violated.

\subsection{Model Specification}

Our model for observables decomposes into a treatment model and an outcome given treatment model, i.e., $P(Y,T\mid Z, \X) = P(T\mid Z, \X)P(Y \mid T, Z, \X)$. We assign each of these a probit BART prior. For the treatment model, randomization of treatment assignment and monotonicity of compliance imply that $\Pr(T=1\mid Z=1, \X) \geq \Pr(T=1\mid Z=0, \X)$ for all $\X$ (see equations \eqref{eq:mon-1} and \eqref{eq:mon-2}). We enforce this constraint by rejecting samples from BART where this condition fails at any point in covariate space. More elaborate approaches to enforcing monotonicity are possible but beyond the scope of the present paper. %As we are not imposing any exclusion restrictions, there are no constraints on our model for the outcome given the treatment and instrument. 

\subsubsection{Partially identified parameters}

Recall that we have two pairs of unidentified parameters,  $(\gamma^{00}_c, \gamma^{00}_n)$ and $(\gamma^{11}_c,\gamma^{11}_a)$. Fixing one element of each pair would solve the identification problem, so we can take $\theta = (\gamma^{00}_n,\gamma^{11}_a)$ without loss of generality. 
%Other parameterizations of $\theta$ are of course possible, but this choice will be convenient for prior specification. 
This is in contrast to \cite{Hirano2000}, who specify a strongly parametric probability model for all four of the unidentified parameters.

We consider three priors on $\theta$. All three are of the form
\begin{equation}
(\mbox{logit}\{\gamma^{00}_n(\X)\}, \mbox{logit}\{\gamma^{11}_a(\X)\})' = \mu\{\phi(\X)\} + h(\X)\beta + \epsilon(x)\label{eq:theta-3}.
\end{equation}
with $\mu(\phi(\X)) = (\mbox{logit}\{\gamma^{01}_n(\X)\}, \mbox{logit}\{\gamma^{10}_a(\X)\})'$, $h(\X)=1$ and $\beta=(b_a, -b_n)$. This centers our prior at a proportional odds model, where the reminder increases the odds of a positive outcome by a factor of $\exp(b_a)$ or $\exp(b_n)$ in always or never takers (respectively) at any covariate value. A natural way to complete this prior is to take $b_s\sim N(0, \sigma_s^2)$ for $s=a,n$ which centers the prior at the exclusion restrictions and expresses prior beliefs about plausible effect sizes through $\sigma_s^2$. For illustration we take $\sigma_s=0.1$ or $0.25$ for the current application. \cite{Hirano2000} estimate principal strata-independent total effects of COPD around -0.35 on the log odds scale, so the more diffuse prior covers a plausible range of possible effect sizes for the direct effect of a reminder within non-compliers.  We would expect any direct beneficial effect of the reminder on the subsequent hospitalization to be smaller than the detrimental effect of a serious chronic disease like COPD purely on substantive grounds.

In the flu application we also have some prior information about likely effect directions, which we can also incorporate in the prior. 
%As observed by \cite{Hirano2000}, 
Any direct effect from the reminder is most likely to be positive, since the reminder probably encourages doctors and patients to take other preventative measures beyond the vaccine. Additionally, \cite{Hirano2000} speculate that the exclusion restriction for never takers is more plausible than for always takers since perceived risk is a key driver of compliance behavior, with low-risk patients more likely to be never takers. A more nuanced view is that the direct effect should be \emph{larger} for always takers than never takers --- even though never takers probably have lower risk on average, we should not rule out the possibility of high-risk never takers who refuse the vaccine due to cost, safety or other concerns. 

A prior for $\theta$ that reflects these beliefs is $(b_a, b_n)\sim \N(b_0, \Sigma_b)\mathbb{1}(b_a>0, b_n>0)$. For the analysis in the sequel we will take $b_0 = (0.05, 0.0)'$, $\Sigma_b = \mbox{diag}(0.13^2, 0.05^2)$. In additional simulations we find that results are insensitive to plausible values of $\mbox{Cov}(b_a, b_n)$. These particular numerical values were chosen  The prior mode is $b_0$, the prior mean is about $(0.125, 0.04)$, and the marginal $90^{th}$ percentile is about 0.25 for $b_a$ and 0.08 for $b_n$. 
%This prior is calibrated so that the direct effect in any takers is larger than that for never takers and both are positive. 
The prior scale for $b_a$ is calibrated so that (with high probability) $b_a$ is smaller in magnitude than the effect of COPD on the hospitalization as reported by \cite{Hirano2000} (the posterior mean was generally around -0.35, SD 0.15). We will call this the ``informed" prior.
For all three priors we set $v=0.025$. 
%$v(x)$ as 
%\begin{equation}
%v(x, \phi) = \{0.025[1 + 200\delta_{x}]\}^2
%\end{equation}
%where 
%$
%\delta_{x} =
%  %\begin{cases}
%   %0 & \text{if } a(\phi(x)) < m(\X^*_j) < b(\phi(x))) \\
%   \max\{0, a(\phi(x))-m(x),\ m(x)-b(\phi(x))\}      %& \text{otherwise}  \end{cases}
%$.

%Even leaving aside this additional information, it is hard to imagine the hypothesized mechanisms for the direct effect  having effects larger than 25 or 30\%, so this prior seems  reasonable.

%
%We describe prior specification for $\gamma^{11}_a(x)$ since the prior on $\gamma^{00}_n(x)$ will be specified similarly. Let $\eta_a^{11}(x)=\logit(\gamma^{11}_a(x))$. We induce a prior on $\gamma_a^{11}$ by assuming a Gaussian process prior on $\eta_a^{11}$:
%\begin{equation}
%\left(\eta_a^{11}(x_1), \eta_a^{11}(x_2),\dots,\eta_a^{11}(x_q)\right)'\sim N((m_{A}(x_1), m_{A}(x_2),\dots,m_{A}(x_q))', \tau_a\Sigma_a(x_1, x_2,\dots,x_q))
%\end{equation}
%
%for some mean function $m$ and covariance function $\Sigma$, where $x_1,x_2,\dots x_q$ are design points of interest. For inference on sample average treatment effects these should be the distinct covariate values observed in the dataset. The scale parameter $\tau_a$ expresses our overall confidence in the specification of the mean function and could also vary with $x$ if appropriate. Since we are primarily interested in $ITT_c$, an additive function of $\gamma^{11}_a(x)$ and $\gamma^{00}_n(x)$, there is little benefit to enforcing smoothness in $\gamma^{11}_a$ or $\gamma^{00}_n(x)$ so we simply take $\Sigma(x_1, x_2,\dots,x_q) = \tau_a^2I$. 
%
%Any number of mean functions are possible. One natural choice is 
%
%\begin{equation}
%m_a(x) = a_a + \logit(\gamma^{10}_a(x)),\label{eq:propoddsA}
%\end{equation}
%
%which centers our prior on a constant proportional odds model (the reminder increases the odds by a multiplicitive factor of $e^{\alpha_a}$ at any covariate value). The value of $\alpha_a$ can be varied over a range of plausible values, or given an informative prior itself. The conditional prior on $m_n$ will be similar:
%\begin{equation}
%m_n(x) = -a_n + \logit(\gamma^{01}_n(x)),\label{eq:propoddsN}
%\end{equation}
%where the negative intercept is to keep $\alpha_a$ and $\alpha_n$ consistent in sign (positive values indicating a protective effect of the reminder).
%
\subsection{Results}

We fit the model described in the previous section to the flu vaccine data, using age and COPD as covariates. Figure \ref{fig:psmembership} shows the probability of belonging to each principal stratum as a function of age and COPD along with marginal 90\% credible intervals. We find a fairly sharp break in compliance behavior at age 65 (the probability of being a never-taker drops, and seems to be shifted largely to always takers), which appears to hold regardless of COPD status. Possible explanations include patients or providers giving more weight to age-based vaccination guidelines, or better insurance coverage and increased access to services in the older cohort. 

Figure \ref{fig:outcometz} shows the outcome distributions by age, COPD, and the treatment assigned and received. There is clear evidence of an age/COPD interaction; this is due at least in part to the study design, where all participants under 65 have at least one chronic disease (possibly COPD). This also means that the 65+ population is on average less likely to he hospitalized than the younger cohort, explaining the seemingly paradoxical decrease in the estimated probability of hospitalization at age 65 in the ``No COPD" group.

\begin{figure}
\begin{center}
\includegraphics[width=5in]{flu-figure/PSMembershipTrunc.pdf}
\caption{Principal strata memberhsip probabilities by age and COPD, including marginal 90\% credible intervals}\label{fig:psmembership}
\end{center}
\end{figure}

\begin{figure}
\begin{center}
\includegraphics[width=3.5in]{flu-figure/OutcomeByTZ.pdf}
\caption{Log odds of a positive outcome (no hospitalization) by age, COPD, and treatment assignment/receipt}\label{fig:outcometz}
\end{center}
\end{figure}


\subsubsection{Causal effects}
We are primarily interested in (partially identified) sample causal effects. 
%Recall that for each unit we observe $T_i(Z_i)$ and $Y_i(T_i(Z_i), Z_i)$, but individual level causal effects (and their averages) are defined in terms of contrasts between potential outcomes; for example, the individual \emph{intent to treat} (ITT) effect for unit $i$, the total effect of the instrument on the response, is $Y_i(T_i(1), 1) - Y_i(T_i(0), 0)$. 
As in \cite{Hirano2000} we will consider estimating the intention-to-treat (ITT) effect in each principal stratum:
\begin{equation}
ITT_s = \frac{1}{n_s}\sum_{i: S_i=s} (Y_i(T_i(1), 1) - Y_i(T_i(0), 0)). 
\end{equation}
where $n_s$ is the number of observations with compliance type $S$. Given a sample from the marginal distribution for $\phi$, and a sample from $\theta$, we can impute each observation's missing principal strata membership and the unobserved potential outcome. With the completed data it is straightforward to compute the sample ITT effects. Computational details are provided in Appendix \ref{app:postmis}

%We also fit the BART model using the full set of covariates in the flu data, which also include race, sex, and indicators for other chronic conditions (diabetes and heart, liver, and kidney disease). \cite{Hirano2000} choose baseline variables based on imbalance in the two $T$ arms, but any variable which predicts compliance behavior or hospitalization risk has the potential to tighten the bounds on $\theta$ (see \cite{Long2013} and the references therein for an asymptotic argument). Note that this is an argument for incorporating baseline covariates that predict the outcome \emph{or} have a significant interaction with $Z$ in the treatment model, rather than basing variable inclusion on balance with respect to $T$. 

%The treatment model is much more discriminative with the extra variables, and it turns out that this is due largely to race (Figure \ref{fig:flupc}). Significant differences in vaccine uptake among different racial/ethnic groups have been observed for some time, even after controlling for age and other risk factors ((cites)), so this result is somewhat unsurprising.
%
%\begin{figure}
%\begin{center}
%\includegraphics[width=4in]{flu-figure/flupc.pdf}
%\caption{Posterior mean estimates of $\pi_c(x)$ from the BART treatment model with age/COPD and the full set of covariates}
%\end{center}
%\label{fig:flupc} 
%\end{figure}

We compare results under our three priors to three models from \cite{Hirano2000}: the model with no exclusion restrictions (``none"), both exclusion restrictions (``both"), or the never-taker exclusion restriction (``n"). The ``Hirano (none)" model has very wide standard deviations, which are driven by their use of diffuse, ``off-the-shelf" priors.  Their marginal prior for the direct effect of the reminder is approximately normal with mean zero and standard deviation 1.5, which puts significant prior probability on implausible values such as large and/or negative direct effects. Such vague priors are inappropriate for partially identified parameters.

In contrast, the BART models all give similar results. The ``BART (0.1)" and ``BART (0.25)" models differ mainly in the width of the posterior standard errors, and then only slightly. The ``BART (0.25)" model assumes that with high probability the magnitude of any direct effect on the log odds is within $\pm 0.5$ -- compare this to the COPD effect, which is estimated to increase the log odds of hospitalization by about 0.35. The ``informed" prior restricts the population effects to be positive but small, which tends to shrink the $ITT_c$ effect toward zero -- the overall $ITT$ effect is identified, so positive effects in the other principal strata lead necessarily to smaller $ITT_c$ estimates than unrestricted models.

The substantive conclusion is largely unchanged: there is only modest evidence for the effectiveness of the vaccine, particularly if we assume the direct effect of the reminder is similar in always-takers and compliers. This is unsurprising given the sample size of $n=2,861$, weakness of the encouragement (Fig. \ref{fig:psmembership}), and relative rarity of the outcome (about 8\% of the study participants were hospitalized). However, unlike \cite{Hirano2000} we conclude that the $ITT_c$ effect is actually fairly robust to plausible deviations from the exclusion restrictions.

%In contrast, the standard deviation of the $ITT_c$ effect in the ``BART (age/COPD)" model is comparable to the point identified ``Hirano (both)" model, despite making no strong assumptions about the functional form of the observable joint distribution (unlike \cite{Hirano2000}) and allowing for deviations from the exclusion restrictions. The estimate of $ITT_c$ is apparently robust to reasonable deviations from the exclusion restrictions. The substantive conclusion from the age/COPD model changes little, however: Assuming the direct effect of the reminder is similar in always-takers and compliers, there is only modest evidence for the efficacy of the flu vaccine. The evidence from the all-covariate model is somewhat stronger in favor of the vaccine. The posterior mean effect is notably larger (0.114 vs 0.086), with a smaller standard deviation (0.064 vs 0.072) while the always- and never-taker effects change very little. 

\begin{figure}
\begin{center} 
\includegraphics[width=5.25in]{flu-figure/flures.pdf}
\caption{Posterior mean and standard deviations for the sample ITT effects in each principal stratum. ``BART (0.1)" and ``BART (0.25)" use the conditional prior centered at the exclusion restrictions with $\sigma_a=\sigma_n=0.1$ or $0.25$, respectively. ``BART (informed)" includes all prior information. The ``Hirano" models are from \cite{Hirano2000}; the ``n" model assumes the exclusion restriction in never-takers, the ``both" model imposes both exclusion restrictions and the ``none" model has no exclusion restrictions.}\label{fig:flures}  
\end{center}
\end{figure}


%Our prior is carefully constructed to represent scientifically plausible states of the world, unlike the ``off-the-shelf" prior proposed in \cite{Hirano2000}. Their marginal prior for the direct effects is approximately normal with a mean of zero and standard deviation 1.5, which puts significant prior probability on implausible values such as large, negative direct effects. These vague priors are not generally good practice in partially identified problems and are at least part of the reason why the authors find little evidence of a positive effect of the vaccine.

%why posterior variance go down bro?
 
%We could go further and let
%\begin{equation}
%m_a(x) = \alpha_a + x'\beta_a + \logit(\gamma^{10}_a(x)),
%\end{equation}
%perhaps fixing some subset of $\beta$ to be identically zero and either setting the rest at plausible values or assigning them prior distributions. Note that the linear term $x'\beta$ should be interpreted as an interaction between covariates and treatment assignment, since we have included $\logit(\gamma^{10}_a(x))$ in the mean function. 



==> JASA_revised copy/flu_ArXiV.tex <==
%!TEX root = HahnMurrayManolopoulou_ArXiV.tex

Our data come from a randomized encouragement study of the effectiveness of an influenza vaccine conducted at an academic primary care practice affiliated with a large teaching hospital in an urban setting \citep{McDonald1992}. Physicians were randomly assigned to treatment or control groups, with treated physicians receiving a computerized reminder about the vaccine when a patient with a scheduled visit also met the U.S. Public Health Service Criteria for receiving a flu vaccine. Patients were eligible for the vaccine if they were 65 or older, or if they had certain severe chronic diseases including chronic obstructive pulmonary disease (COPD).
% lung disease, asthma, diabetes, congestive heart failure, or severe liver or kidney failure. 
The outcome of interest is subsequent hospitalization for flu-related illness, and the covariates include the patient's age and COPD status. \cite{Hirano2000} conduct a Bayesian analysis of this problem, placing a default joint prior over all the identified and unidentified parameters. In this application we perform an alternative selectively informative analysis with modular priors. %One aspect of this design which has been ignored to date is that the inclusion criteria potentially induce a sharp change in the probability of a positive outcome at age 65, since anyone 65 or older was in the study population while a 64 year-old patient would only be included if he or she had a serious, chronic disease.
We will use the terms ``reminder'', ``instrument'' and ``encouragement'' interchangably here, prefering ``reminder'' in the context of the specific applied problem.
 
\subsection{Causal Inference in a Binary Instrumental Variables Model}
%\sayan{fix to make everything conditional on X (doesn't change anything substantively)} 

Let $Z_i, T_i$, and $Y_i$ be the observed values of the treatment assignment (or encouragement, or instrument), treatment received, and outcome for observation $i$, respectively.  Let $X_i$ be a vector of baseline covariates. In the flu data, $Z_i=1$ if encouragement (the reminder) was administered, $T_i=1$ if the vaccine was administered, and $Y_i=1$ if the patient was \emph{not} hospitalized. As in \cite{Angrist1996} and \cite{Hirano2000} define the \emph{potential outcomes} $T_i(z)$ and $ Y_i(t,z)$ as the treatment
assignment that would have been observed had we fixed $Z_i=z$ and the outcome we would have observed fixing $T_i=t, Z_i=z$, respectively. We will suppress indexing by $i$ for population quantities. We make the stable unit treatment value assumption (SUTVA) \citep{Angrist1996}, i.e. that there is no interference between units and no alternative versions of treatment. \footnote{\cite{Hirano2000} point out that in an infectious disease application with individuals as the unit of randomization this assumption is unlikely to hold exactly, but constitutes a reasonable first order approximation.} Mathematically, SUTVA implies that $T_i(\mathbf{z})=T_i(z_i)$ and $Y_i(\mathbf{t}, \mathbf{z})=Y_i(t_i, z_i)$, where $\mathbf{z}, \mathbf{t}$ are vectors of instrument/encouragement assignment and treatments received (respectively) for the entire sample.

In this application the complete vector of binary response variables is 
\begin{equation}
U_i=(T_i(0), T_i(1), Y_i(0,0), Y_i(0,1), Y_i(1,0), Y_i(1,1))',
\end{equation}
 the collection of treatments and outcomes under all possible experimental conditions. However, we observe only $T_i\equiv T_i(Z_i)$ and $Y_i\equiv Y_i(T_i(Z_i), Z_i)$, where $Z_i$ is randomly assigned at the study outset. 
%
%as follows:
%\begin{equation}
%T_i = Z_iT_i(1) + (1-Z_i)T_i(0)
%\end{equation}
%\begin{equation}
% Y_i = T_iZ_iY_i(1,1) + 
%(1-T_i)Z_iY_i(0,1) + 
%T_i(1-Z_i)Y_i(1,0) + 
%(1-T_i)(1-Z_i)Y_i(0,0).
%\end{equation}
%
We can define compliance types or principal strata $S$ based on the possible values for $(T(1), T(0))$ -- see Table \ref{tab:comptype}. 
%
\begin{table}
\begin{center}
    \begin{tabular}{cc|ll}
        $T(1)$ & $T(0)$ & $S$ (Compliance Type) & ~    \\ \hline
        0     & 0     & Never Taker     & (n) \\ 
        1     & 1     & Always Taker    & (a) \\ 
        1     & 0     & Complier        & (c) \\ 
        0     & 1     & Defier          & (d) \\
    \end{tabular}
  \caption{Compliance types, or principal strata, defined by response patterns across levels of $Z$.}
  \label{tab:comptype}
  \end{center}
\end{table}
%
We will assume that the encouragement $Z$ is ignorable or randomly assigned (as it is in the flu data).
We also assume that there are no defiers (``monotonicity of compliance"), i.e., $ \Pr(S=d\mid \X)=0$. In the current setting a defier would be a patient who would \emph{only} receive the vaccine if the reminder was \emph{not} administered, which is quite unlikely.

Let $\pi_s(x) = \Pr(S=s\mid \X)$  and 
$\gamma^{tz}_s(x) = \Pr( Y(t,z)=1\mid S=s, \X)$ denote the principal strata and potential outcome probability models. Under the above assumptions the potential outcome and principal strata distributions are linked to the joint distribution of observables by the following equations.
%
\begin{align}
\Pr(T=1\mid Z=0, \X) &= \pi_a(\X)\label{eq:mon-1},\\
\Pr(T=1\mid Z=1, \X) &= \pi_c(\X) + \pi_a(\X)\label{eq:mon-2},\\
\Pr(Y=1\mid T=0, Z=0, \X) &= [\pi_c(\X)\gamma^{00}_c(\X) + \pi_n(\X)\gamma^{00}_n(\X)]/[\pi_c(\X) + \pi_n(\X)]\label{eq:mon-3},\\
\Pr(Y=1\mid T=1, Z=1, \X) &= [\pi_c(\X)\gamma^{11}_c(\X) + \pi_a(\X)\gamma^{11}_a(\X)]/[\pi_c(\X) + \pi_a(\X)]\label{eq:mon-4},\\
\Pr(Y=1\mid T=0, Z=1, \X) &= \gamma^{01}_n(\X),\\
\Pr(Y=1\mid T=1, Z=0, \X) &= \gamma^{10}_a(\X)\label{eq:mon-last}.
\end{align}
\cite{Richardson2010} derive this mixture relationship between principal strata/potential outcome distributions and the observable joint in detail under a range of assumptions about the latent variables (see also \cite{Imbens1997a} and \cite{Richardson2011}).

The probabilities on the left hand side completely determine the joint distribution of observables ($Y$ and $T$ given $Z$) and hence constitute a basis for $\phi$. Clearly $\pi$, $\gamma^{01}_n$ and $\gamma^{10}_a$ are one-to-one maps from $\phi$, and are point identified as well. However, $\gamma^{00}_c,\ \gamma^{00}_n,\ \gamma^{11}_c,$ and $ \gamma^{11}_a$ are not. For example, at any point in covariate space $\gamma^{11}_c(x)$ and $\gamma^{11}_a(x)$ must lie on the line segment given by the intersection of the line in equation \eqref{eq:mon-4} and $[0,1]\times [0,1]$, but the data are wholly uninformative about their position on that line segment. In particular, the range of $\gamma^{11}_a(x)$ is

\begin{equation}
\left(
	\min\left(
		0, \frac{\pi_a(x)+\pi_c(x)}{\pi_a(x)}p_{1\mid 11}(x) - \frac{\pi_c(x)}{\pi_a(x)}
	\right),\,
	\max\left(
		1, \frac{\pi_a(x)+\pi_c(x)}{\pi_a(x)}p_{1\mid 11}(x)
	\right)
\right)\label{eq:gbound}
\end{equation}
where $p_{1\mid 11}(x) = \Pr(Y=1\mid T=1, Z=1,\X)$. The situation is exactly the same for $\gamma^{00}_c(x)$ and $\gamma^{00}_n(x)$, with the line given by \eqref{eq:mon-3} and bounds similar to \eqref{eq:gbound} (large sample bounds on causal effects within principal strata were introduced by  \cite{zhang2003estimation}; see \cite{Richardson2011} for bounds under monotonicity and other assumptions, as well as further references).

%j 7/29
%In the instrumental variables literature, 
Point identification for the remaining parameters is often obtained through further assumptions on the distribution of the potential outcomes. The \emph{stochastic exclusion restriction} for compliance type $s$ posits that there is no direct effect of $Z$ on $Y$; that is, $\gamma^{i0}_s = \gamma^{i1}_s$ for $i=0,1$ \citep{Hirano2000}. From \eqref{eq:mon-1}-\eqref{eq:mon-last} it is clear that this achieves point identification for the entire distribution of the potential outcomes.

\cite{Hirano2000} anticipated failures of the exclusion restrictions, noting that a reminder about flu shots might also prompt physicians to counsel patients about other preventative measures to avoid contracting the flu. They propose relaxing the exclusion restrictions and resolving the resulting nonidentifiability through prior probability modeling. In this sense our approach and theirs are philosophically similar, but our framework affords us significant flexibility in choosing the model for $\phi$ while transparently embedding prior information about $\theta$, which is difficult to do in their modeling setup. In our subsequent analysis we will avoid imposing any exclusion restrictions.
%
% What will be particularly relevant for our  analysis is that any direct effect of the reminder on subsequent hospitalization for flu-related illness should be positive and relatively small, and is likely to be larger in always takers than in never takers (since one factor driving uptake of the vaccine and other prophylactic measures is perceived risk, which is higher in always takers).
%
%
%
%
%
%Our focus will be on \emph{intention-to-treat (ITT)} effects. The sample ITT effect is 
%
%\begin{equation}
%ITT = \frac{1}{n}\sum_{i=1}^n (Y_i(T_i(1), 1) - Y_i(T_i(0), 0)). 
%\end{equation}
%Sample ITT effects for different compliance types are defined similarly:
%\begin{equation}
%ITT_s = \frac{1}{n_s}\sum_{i: S_i=s} (Y_i(T_i(1), 1) - Y_i(T_i(0), 0)). 
%\end{equation}
%where $n_s$ is the number of observations with compliance type $S$ \citep{Hirano2000}. 
%The potential outcome distributions $\gamma$ and compliance type distributions $\pi$ are linked to the joint distribution of observables by the following equations (suppressing the dependence on $x$):
%
%\begin{align}
%\Pr(T=1\mid Z=0) &= \pi_D + \pi_a\\
%\Pr(T=1\mid Z=1) &= \pi_c + \pi_a\\
%\Pr(Y=1\mid T=0, Z=0) &= (\pi_c\gamma^{00}_c + \pi_n\gamma^{00}_n)/(\pi_c + \pi_n)\\
%\Pr(Y=1\mid T=1, Z=1) &= (\pi_c\gamma^{11}_c + \pi_a\gamma^{11}_a)/(\pi_c + \pi_a)\\
%\Pr(Y=1\mid T=0, Z=1) &= (\pi_D\gamma^{01}_D + \pi_n\gamma^{01}_n)/(\pi_D + \pi_n)\\
%\Pr(Y=1\mid T=1, Z=0) &= (\pi_D\gamma^{10}_D + \pi_a\gamma^{10}_a)/(\pi_D + \pi_a).
%\end{align}
%
% Assuming the exclusion restriction in always and never takers point identifies the (population) intent to treat effect in compliers:
%\begin{equation}
%PITT_{C} = \gamma^{11}_c - \gamma^{00}_c,
%\end{equation}
%which is equivalent to the local average treatment effect (LATE) if the exclusion restriction holds in compliers as well \cite{Angrist1996}. In the absence of the exclusion restrictions for always takers and/or compliers, $PITT_c$ is bounded by the equations above and the fact that the $\gamma$'s are probabilities. Since the data are informative about these bounds (the bounds themselves are point identified) $PITT_c$ is \emph{partially} identified.
%
%There are theoretical and empirical reasons to suspect that the exclusion restrictions might be violated. \cite{Richardson2011} give a detailed exposition of bounds on the joint distribution of $(Y, T\mid Z)$ induced by assuming various combinations of monotonicity and the exclusion restrictions.  \cite{Richardson2011} compute posterior distributions of these bounds under a Dirichlet-multinomial model without covariates. Assuming monotonicity, they find that the posterior probability of violating the bounds is 0.54 and 0.06 for the exclusion restriction in always takers and never takers respectively. Since the bounds are necessary but not sufficient for the exclusion restrictions to hold, there is ample evidence that the exclusion restrictions are violated.

\subsection{Model Specification}

Our model for observables decomposes into a treatment model and an outcome given treatment model, i.e., $P(Y,T\mid Z, \X) = P(T\mid Z, \X)P(Y \mid T, Z, \X)$. We assign each of these a probit BART prior. For the treatment model, randomization of treatment assignment and monotonicity of compliance imply that $\Pr(T=1\mid Z=1, \X) \geq \Pr(T=1\mid Z=0, \X)$ for all $\X$ (see equations \eqref{eq:mon-1} and \eqref{eq:mon-2}). We enforce this constraint by rejecting samples from BART where this condition fails at any point in covariate space. More elaborate approaches to enforcing monotonicity are possible but beyond the scope of the present paper. %As we are not imposing any exclusion restrictions, there are no constraints on our model for the outcome given the treatment and instrument. 

\subsubsection{Partially identified parameters}

Recall that we have two pairs of unidentified parameters,  $(\gamma^{00}_c, \gamma^{00}_n)$ and $(\gamma^{11}_c,\gamma^{11}_a)$. Fixing one element of each pair would solve the identification problem, so we can take $\theta = (\gamma^{00}_n,\gamma^{11}_a)$ without loss of generality. 
%Other parameterizations of $\theta$ are of course possible, but this choice will be convenient for prior specification. 
This is in contrast to \cite{Hirano2000}, who specify a strongly parametric probability model for all four of the unidentified parameters.

We consider three priors on $\theta$. All three are of the form
\begin{equation}
(\mbox{logit}\{\gamma^{00}_n(\X)\}, \mbox{logit}\{\gamma^{11}_a(\X)\})' = \mu\{\phi(\X)\} + h(\X)\beta + \epsilon(x)\label{eq:theta-3}.
\end{equation}
with $\mu(\phi(\X)) = (\mbox{logit}\{\gamma^{01}_n(\X)\}, \mbox{logit}\{\gamma^{10}_a(\X)\})'$, $h(\X)=1$ and $\beta=(b_a, -b_n)$. This centers our prior at a proportional odds model, where the reminder increases the odds of a positive outcome by a factor of $\exp(b_a)$ or $\exp(b_n)$ in always or never takers (respectively) at any covariate value. A natural way to complete this prior is to take $b_s\sim N(0, \sigma_s^2)$ for $s=a,n$ which centers the prior at the exclusion restrictions and expresses prior beliefs about plausible effect sizes through $\sigma_s^2$. For illustration we take $\sigma_s=0.1$ or $0.25$ for the current application. \cite{Hirano2000} estimate principal strata-independent total effects of COPD around -0.35 on the log odds scale, so the more diffuse prior covers a plausible range of possible effect sizes for the direct effect of a reminder within non-compliers.  We would expect any direct beneficial effect of the reminder on the subsequent hospitalization to be smaller than the detrimental effect of a serious chronic disease like COPD purely on substantive grounds.

In the flu application we also have some prior information about likely effect directions, which we can also incorporate in the prior. 
%As observed by \cite{Hirano2000}, 
Any direct effect from the reminder is most likely to be positive, since the reminder probably encourages doctors and patients to take other preventative measures beyond the vaccine. Additionally, \cite{Hirano2000} speculate that the exclusion restriction for never takers is more plausible than for always takers since perceived risk is a key driver of compliance behavior, with low-risk patients more likely to be never takers. A more nuanced view is that the direct effect should be \emph{larger} for always takers than never takers --- even though never takers probably have lower risk on average, we should not rule out the possibility of high-risk never takers who refuse the vaccine due to cost, safety or other concerns. 

A prior for $\theta$ that reflects these beliefs is $(b_a, b_n)\sim \N(b_0, \Sigma_b)\mathbb{1}(b_a>0, b_n>0)$. For the analysis in the sequel we will take $b_0 = (0.05, 0.0)'$, $\Sigma_b = \mbox{diag}(0.13^2, 0.05^2)$. In additional simulations we find that results are insensitive to plausible values of $\mbox{Cov}(b_a, b_n)$. These particular numerical values were chosen  The prior mode is $b_0$, the prior mean is about $(0.125, 0.04)$, and the marginal $90^{th}$ percentile is about 0.25 for $b_a$ and 0.08 for $b_n$. 
%This prior is calibrated so that the direct effect in any takers is larger than that for never takers and both are positive. 
The prior scale for $b_a$ is calibrated so that (with high probability) $b_a$ is smaller in magnitude than the effect of COPD on the hospitalization as reported by \cite{Hirano2000} (the posterior mean was generally around -0.35, SD 0.15). We will call this the ``informed" prior.
For all three priors we set $v=0.025$. 
%$v(x)$ as 
%\begin{equation}
%v(x, \phi) = \{0.025[1 + 200\delta_{x}]\}^2
%\end{equation}
%where 
%$
%\delta_{x} =
%  %\begin{cases}
%   %0 & \text{if } a(\phi(x)) < m(\X^*_j) < b(\phi(x))) \\
%   \max\{0, a(\phi(x))-m(x),\ m(x)-b(\phi(x))\}      %& \text{otherwise}  \end{cases}
%$.

%Even leaving aside this additional information, it is hard to imagine the hypothesized mechanisms for the direct effect  having effects larger than 25 or 30\%, so this prior seems  reasonable.

%
%We describe prior specification for $\gamma^{11}_a(x)$ since the prior on $\gamma^{00}_n(x)$ will be specified similarly. Let $\eta_a^{11}(x)=\logit(\gamma^{11}_a(x))$. We induce a prior on $\gamma_a^{11}$ by assuming a Gaussian process prior on $\eta_a^{11}$:
%\begin{equation}
%\left(\eta_a^{11}(x_1), \eta_a^{11}(x_2),\dots,\eta_a^{11}(x_q)\right)'\sim N((m_{A}(x_1), m_{A}(x_2),\dots,m_{A}(x_q))', \tau_a\Sigma_a(x_1, x_2,\dots,x_q))
%\end{equation}
%
%for some mean function $m$ and covariance function $\Sigma$, where $x_1,x_2,\dots x_q$ are design points of interest. For inference on sample average treatment effects these should be the distinct covariate values observed in the dataset. The scale parameter $\tau_a$ expresses our overall confidence in the specification of the mean function and could also vary with $x$ if appropriate. Since we are primarily interested in $ITT_c$, an additive function of $\gamma^{11}_a(x)$ and $\gamma^{00}_n(x)$, there is little benefit to enforcing smoothness in $\gamma^{11}_a$ or $\gamma^{00}_n(x)$ so we simply take $\Sigma(x_1, x_2,\dots,x_q) = \tau_a^2I$. 
%
%Any number of mean functions are possible. One natural choice is 
%
%\begin{equation}
%m_a(x) = a_a + \logit(\gamma^{10}_a(x)),\label{eq:propoddsA}
%\end{equation}
%
%which centers our prior on a constant proportional odds model (the reminder increases the odds by a multiplicitive factor of $e^{\alpha_a}$ at any covariate value). The value of $\alpha_a$ can be varied over a range of plausible values, or given an informative prior itself. The conditional prior on $m_n$ will be similar:
%\begin{equation}
%m_n(x) = -a_n + \logit(\gamma^{01}_n(x)),\label{eq:propoddsN}
%\end{equation}
%where the negative intercept is to keep $\alpha_a$ and $\alpha_n$ consistent in sign (positive values indicating a protective effect of the reminder).
%
\subsection{Results}

We fit the model described in the previous section to the flu vaccine data, using age and COPD as covariates. Figure \ref{fig:psmembership} shows the probability of belonging to each principal stratum as a function of age and COPD along with marginal 90\% credible intervals. We find a fairly sharp break in compliance behavior at age 65 (the probability of being a never-taker drops, and seems to be shifted largely to always takers), which appears to hold regardless of COPD status. Possible explanations include patients or providers giving more weight to age-based vaccination guidelines, or better insurance coverage and increased access to services in the older cohort. 

Figure \ref{fig:outcometz} shows the outcome distributions by age, COPD, and the treatment assigned and received. There is clear evidence of an age/COPD interaction; this is due at least in part to the study design, where all participants under 65 have at least one chronic disease (possibly COPD). This also means that the 65+ population is on average less likely to he hospitalized than the younger cohort, explaining the seemingly paradoxical decrease in the estimated probability of hospitalization at age 65 in the ``No COPD" group.

\begin{figure}
\begin{center}
\includegraphics[width=5in]{flu-figure/PSMembershipTrunc.pdf}
\caption{Principal strata memberhsip probabilities by age and COPD, including marginal 90\% credible intervals}\label{fig:psmembership}
\end{center}
\end{figure}

\begin{figure}
\begin{center}
\includegraphics[width=3.5in]{flu-figure/OutcomeByTZ.pdf}
\caption{Log odds of a positive outcome (no hospitalization) by age, COPD, and treatment assignment/receipt}\label{fig:outcometz}
\end{center}
\end{figure}


\subsubsection{Causal effects}
We are primarily interested in (partially identified) sample causal effects. 
%Recall that for each unit we observe $T_i(Z_i)$ and $Y_i(T_i(Z_i), Z_i)$, but individual level causal effects (and their averages) are defined in terms of contrasts between potential outcomes; for example, the individual \emph{intent to treat} (ITT) effect for unit $i$, the total effect of the instrument on the response, is $Y_i(T_i(1), 1) - Y_i(T_i(0), 0)$. 
As in \cite{Hirano2000} we will consider estimating the intention-to-treat (ITT) effect in each principal stratum:
\begin{equation}
ITT_s = \frac{1}{n_s}\sum_{i: S_i=s} (Y_i(T_i(1), 1) - Y_i(T_i(0), 0)). 
\end{equation}
where $n_s$ is the number of observations with compliance type $S$. Given a sample from the marginal distribution for $\phi$, and a sample from $\theta$, we can impute each observation's missing principal strata membership and the unobserved potential outcome. With the completed data it is straightforward to compute the sample ITT effects. Computational details are provided in Appendix \ref{app:postmis}

%We also fit the BART model using the full set of covariates in the flu data, which also include race, sex, and indicators for other chronic conditions (diabetes and heart, liver, and kidney disease). \cite{Hirano2000} choose baseline variables based on imbalance in the two $T$ arms, but any variable which predicts compliance behavior or hospitalization risk has the potential to tighten the bounds on $\theta$ (see \cite{Long2013} and the references therein for an asymptotic argument). Note that this is an argument for incorporating baseline covariates that predict the outcome \emph{or} have a significant interaction with $Z$ in the treatment model, rather than basing variable inclusion on balance with respect to $T$. 

%The treatment model is much more discriminative with the extra variables, and it turns out that this is due largely to race (Figure \ref{fig:flupc}). Significant differences in vaccine uptake among different racial/ethnic groups have been observed for some time, even after controlling for age and other risk factors ((cites)), so this result is somewhat unsurprising.
%
%\begin{figure}
%\begin{center}
%\includegraphics[width=4in]{flu-figure/flupc.pdf}
%\caption{Posterior mean estimates of $\pi_c(x)$ from the BART treatment model with age/COPD and the full set of covariates}
%\end{center}
%\label{fig:flupc} 
%\end{figure}

We compare results under our three priors to three models from \cite{Hirano2000}: the model with no exclusion restrictions (``none"), both exclusion restrictions (``both"), or the never-taker exclusion restriction (``n"). The ``Hirano (none)" model has very wide standard deviations, which are driven by their use of diffuse, ``off-the-shelf" priors.  Their marginal prior for the direct effect of the reminder is approximately normal with mean zero and standard deviation 1.5, which puts significant prior probability on implausible values such as large and/or negative direct effects. Such vague priors are inappropriate for partially identified parameters.

In contrast, the BART models all give similar results. The ``BART (0.1)" and ``BART (0.25)" models differ mainly in the width of the posterior standard errors, and then only slightly. The ``BART (0.25)" model assumes that with high probability the magnitude of any direct effect on the log odds is within $\pm 0.5$ -- compare this to the COPD effect, which is estimated to increase the log odds of hospitalization by about 0.35. The ``informed" prior restricts the population effects to be positive but small, which tends to shrink the $ITT_c$ effect toward zero -- the overall $ITT$ effect is identified, so positive effects in the other principal strata lead necessarily to smaller $ITT_c$ estimates than unrestricted models.

The substantive conclusion is largely unchanged: there is only modest evidence for the effectiveness of the vaccine, particularly if we assume the direct effect of the reminder is similar in always-takers and compliers. This is unsurprising given the sample size of $n=2,861$, weakness of the encouragement (Fig. \ref{fig:psmembership}), and relative rarity of the outcome (about 8\% of the study participants were hospitalized). However, unlike \cite{Hirano2000} we conclude that the $ITT_c$ effect is actually fairly robust to plausible deviations from the exclusion restrictions.

%In contrast, the standard deviation of the $ITT_c$ effect in the ``BART (age/COPD)" model is comparable to the point identified ``Hirano (both)" model, despite making no strong assumptions about the functional form of the observable joint distribution (unlike \cite{Hirano2000}) and allowing for deviations from the exclusion restrictions. The estimate of $ITT_c$ is apparently robust to reasonable deviations from the exclusion restrictions. The substantive conclusion from the age/COPD model changes little, however: Assuming the direct effect of the reminder is similar in always-takers and compliers, there is only modest evidence for the efficacy of the flu vaccine. The evidence from the all-covariate model is somewhat stronger in favor of the vaccine. The posterior mean effect is notably larger (0.114 vs 0.086), with a smaller standard deviation (0.064 vs 0.072) while the always- and never-taker effects change very little. 

\begin{figure}
\begin{center} 
\includegraphics[width=5.25in]{flu-figure/flures.pdf}
\caption{Posterior mean and standard deviations for the sample ITT effects in each principal stratum. ``BART (0.1)" and ``BART (0.25)" use the conditional prior centered at the exclusion restrictions with $\sigma_a=\sigma_n=0.1$ or $0.25$, respectively. ``BART (informed)" includes all prior information. The ``Hirano" models are from \cite{Hirano2000}; the ``n" model assumes the exclusion restriction in never-takers, the ``both" model imposes both exclusion restrictions and the ``none" model has no exclusion restrictions.}\label{fig:flures}  
\end{center}
\end{figure}


%Our prior is carefully constructed to represent scientifically plausible states of the world, unlike the ``off-the-shelf" prior proposed in \cite{Hirano2000}. Their marginal prior for the direct effects is approximately normal with a mean of zero and standard deviation 1.5, which puts significant prior probability on implausible values such as large, negative direct effects. These vague priors are not generally good practice in partially identified problems and are at least part of the reason why the authors find little evidence of a positive effect of the vaccine.

%why posterior variance go down bro?
 
%We could go further and let
%\begin{equation}
%m_a(x) = \alpha_a + x'\beta_a + \logit(\gamma^{10}_a(x)),
%\end{equation}
%perhaps fixing some subset of $\beta$ to be identically zero and either setting the rest at plausible values or assigning them prior distributions. Note that the linear term $x'\beta$ should be interpreted as an interaction between covariates and treatment assignment, since we have included $\logit(\gamma^{10}_a(x))$ in the mean function. 



==> JASA_revised copy/partial_ID_lit_review_short.tex <==
A statistical model $p(y\mid\tau)$ indexed by a parameter $\tau\in\Ts$ is said to be {\em identifiable} or {\em identified} if parameter values correspond uniquely to distinct probability distributions over observables. That is, $p(y\mid\tau)=p(y\mid\tau')$ for all $y$ if and only if $\tau=\tau'$. A model that is not identified is simply referred to as unidentified. 
%j 7/29
%Intuitively, in an identified model, the data-generating distribution (as indexed by parameter values) can be uniquely ``identified", given sufficiently many observations. 
The importance of identifiability as a modeling concern has its earliest roots in econometrics, the term first being introduced in \cite{Koopmans1949}.  Other seminal references include \cite{haavelmo1943, haavelmo1944} and \cite{KoopmansReiersol1950}.  Unidentifiability arises naturally in econometric analysis of observational data as a byproduct of imperfect measurement and/or various data censoring mechanisms. 
%j 7/29
%The widely-used errors-in-variables linear model is a textbook example; see \cite{Poirier1998} section 3.4 and the many references therein.   
The Bayesian perspective on identifiability has been comprehensively reviewed in \cite{Aldrich2002} and more recently in \cite{MartinGonzalez2010}. 

The notion of {\em partial identifiability} or {\em partial identification} of parameters expands the concept of identification to consider cases of partial learning. A more general definition of identifiability is $p(y\mid\tau)=p(y\mid\tau')$ if and only if $t(\tau)=t(\tau')$ for some non-constant function $t$; here $t$ is an ``identifying function" in the terminology of \cite{Kadane1975}. When $t$ is one-to-one, we recover the traditional definition of identifiability, or {\em point identification}. When the $t$ with the finest preimage satisfying this condition is many-to-one, the model is partially identified --- the intuition being that asymptotically we can only isolate the value of $t(\tau)$ consistent with the data, which will correspond to a proper subset of $\Ts$ with more than one element. For this reason, and in contrast to point identification, it is common to talk of {\em set identification}. For a more rigorous exposition of the theory of functional identification, refer to \cite{Kadane1975}.
 
%Specifically, partial identification refers to cases where the set of parameter values consistent with an infinite amount of data may be restricted to a proper subset of the a priori set of possible values (though not to a unique value).  In light of this expanded notion, an identified model is one in which parameters are said to be {\em point identified} and a partially identified model is one in which the parameters are merely {\em set identified}.  
Early examples of the partial identification concept include \cite{frisch1934statistical}, \cite{frechet1951tableaux} and \cite{duncan1953alternative}.  In recent years, interest in partial identification has accelerated; an excellent recent review article is \cite{Tamer2010} which includes comprehensive citations. See also the book-length treatments by Manski  \citep{manski1995identification,manski2003partial,manski2007identification}.
%j 7/29
%more comprehensive citations than we do here.  
%
Recent contributions from a Bayesian perspective have focused primarily on asymptotic properties of the posterior distribution over partially identified parameters, notably \cite{gustafson2005model} and \cite{gustafson2010bayesian}. \cite{moon2012bayesian} examine asymptotic discrepancies between Bayesian credible regions and frequentist confidence sets for set-identified parameters.  \cite{florens2011bayesian} consider a theoretical framework for studying posteriors of partially identified parameters in nonparametric models.
%j 7/29
%; they also provide numerous citations of recent developments in econometrics concerning identification and instances of recent Bayesian approaches to a wide range of econometric problems.  
\cite{kline2013default} develop large sample approximations of posterior probabilities that particular parameter values lie in the identified set without reference to a prior on the partially identified parameter.

Our approach differs from these recent contributions in three ways.  One, it is tailored to a nonlinear regression setting with possibly many predictors and complicated inter-relationships; most of the recent literature considers much simpler examples, often without any covariates.  Two, our focus is on practical methods for making inferences on parameters of interest with finite samples; most of the recent literature has focused on theoretical and specifically large-sample issues.  Three, we introduce an efficient computational scheme for sensitivity analysis, an issue which has received relatively little attention in %the recent Bayesian partial identification
the literature.  Most previous work focuses on wholly unidentified parameters and typically requires multiple iterations of model fitting; see e.g. \cite{McCandless2007, Molitor2009} and \cite{McCandless2012} in the context of causal inference/observational data analysis, and \cite{Daniels2008} and chapter 15 of \cite{little1987statistical} for extensive reviews in missing data problems.







==> JASA_revised copy/sec.tex <==
%The goal of our analysis is not to provide a definitive estimate of the fraction of U.S. firms that misreport; indeed a precise estimate will vary depending on the assumptions one brings to the analysis.  Rather our goal is to provide a framework for permitting interested individuals to compare differing conclusions on a common basis, by systematically combining the same data with varying assumptions about the observation process.  To be sure, sensitivity analysis has long been advocated (\cite{Leamer1978}) although in our experience these appeals are more honored in the breach than in the observance.  Our present efforts are intended to make sensitivity analysis as straightforward as possible so that model fitting does not have to be undertaken anew each time an additional observation model is entertained.  Additionally, our approach is to use an exceptionally flexible nonlinear regression method to estimate the identified portion of the model; this is in contrast to the relatively common practice of choosing a model which resolves non-identification in a way that simultaneously restricts the identified portion of the model (perhaps inappropriately).  Examples of this phenomenon are provided in the literature review below.
 

Since 1982, the United States Securities and Exchange Commission (SEC) has released public notices called Accounting and Auditing Enforcement Releases, or AAERs.  AAERs are financial reports ``related to enforcement actions concerning civil lawsuits brought by the Commission in federal court and notices and orders concerning the institution and/or settlement of administrative proceedings"  \citep{SECwebsite}. Informally, AAERs comprise a list of publicly traded firms that the SEC has cited for misconduct in one form or another.  

For brevity, we adopt the nomenclature ``cheating'' and ``caught'', with the understanding that ``cheating" is operationally defined as any accounting anomaly that would lead to an AAER being issued, were it explicitly brought to the SEC's attention.  This interpretation entails that no ``caught" firms did not ``cheat", by definition.

Our goal is to provide an estimate of the prevalence of accounting misconduct in the U.S. economy, defined as all actual (caught) and potential (uncaught) AAERs.  Predicting which companies are likely to cheat, on the basis of observable firm characteristics, is complicated by the fact that there are potentially many instances of misconduct of which the SEC is unaware.  Thus, we do not directly observe which firms cheat, but merely the subset of cheating firms that were {\it caught} doing so.  A naive regression analysis would therefore only speak to the question of which attributes are predictive of getting caught cheating.  To complete the analysis, one must incorporate knowledge or conjectures concerning the impact firm attributes have on the likelihood of misconduct being discovered.  

Problems with similar structure appear in the literature under the heading of ``partially observed binary data".  Regression models for such data have been studied in many different fields, going by various names.  For example, \cite{Lancaster1996} considers the case where the observation model is covariate independent under the name ``contaminated case-control", building on \cite{prentice1979logistic}.  \cite{poirier1980partial} studies such data under the rubric of ``partially observed bivariate probit models", building on the work of \cite{Heckman1976,Heckman1978,Heckman1979}.  Our analysis follows closely the approach taken in \cite{Dyck2013}, where the prevalence of financial misreporting is tackled via several methods, including the bivariate probit model of \cite{poirier1980partial} which was suggested specifically for the securities fraud problem in \cite{Wang2013}.
 
Key references concerning the more general problem of likelihood-based inference in the presence of missing data and/or biased sampling include \cite{rubin1976inference,dawid1977likelihood, little1987statistical, efron1994missing} and \cite{chib2009estimation}, to name but a few.
 
\subsection{Data}
Our data are aggregated from three main sources.  First, the AAER response variable was obtained from the Center for Financial Reporting and Management (CFRM) at Berkeley's Haas School of Business.  Detailed information about the full data set can be found in \cite{dechow2011predicting}. 

Second, additional firm attributes are obtained from the CompuStat North America Annual Fundamentals database via the Wharton Research Data Service (WRDS).  These data are then merged with the AAERs using Global Company Key (GVKEY) by year.  Specifically, the features considered are:
\begin{itemize}\addtolength{\itemsep}{-0.5\baselineskip}
\item fiscal year,
\item cash,
\item net income,
\item capital investments,
\item SIC industry code,
\item qui tam dummy variable.
\end{itemize}
\noindent Cash, net income and capital investments are all recorded as a fraction of the firm's total assets.  Standard industrial classifications are given in terms of ten major divisions, denoted A-J by the Occupational Safety and Health Administration.  The {\em qui tam} dummy variable is derived from the SIC codes; it denotes if a firm is in an industry where persons responsible for revealing misconduct are eligible to receive some part of any award resulting from subsequent prosecution.  Similar to \cite{dyck2008corporate} and  \cite{jayaraman2010whistle}, our qui tam variable is set to one for firms with SIC code 381x, 283x, 37xx, 5122 or 80xx, which includes healthcare providers and pharmaceutical firms, and airplane, missile, and tank manufacturers.  It is reasonable to suppose that firms in these industries have a greater likelihood of any misconduct being exposed as a result of incentivized employees.  

Finally, a keyword search at the Financial Times web page (www.ft.com) was conducted on each company name and the number of search results was recorded by year.  This variable provides a crude measure of media exposure.  Although discrepancies between firm names as recorded in CompuStat and firm names as reported in Financial Times articles lead to measurement error of this variable, it still provides a  reasonable proxy for name recognition and cultural visibility. Most firms will never be mentioned in any news article; a few firms are routinely mentioned in the press. To adjust for the fact that web traffic has increased over that period, we normalize the search results count by the total number of hits across all companies in a given year.

We restrict our analysis to U.S. firms who had positive net income for the given year, considering the period between 2004 and 2010, for a total of $6,641$ unique firms and a total of $n=25,889$ total firm-year observations.

\subsection{Model specification}
%We index our firm-year observations by $i = 1, \dots, n$. 
Let $Z_i$ indicate ``cheating" in firm-year $i$ and let $W_i$ indicate ``getting caught" in firm-year $i$. We assume that with some probability cheaters get caught, but there are no firms who get caught when they are not cheating (this is consistent with our operational definition of ``cheating"). Additonally, the data is ``presence-only'' in that we have no confirmation that any given firm is for sure non-cheating.  We would like to infer $\Pr(Z_i\mid \X)$, which would allow us to compute an aggregate estimate of cheating prevalence over 2004-2010:
\begin{equation}
\alpha \equiv \displaystyle \sum_i \mbox{Pr}(Z_i=1 \mid \X_i) = \displaystyle\sum_i \frac{\mbox{Pr}(Z_i=1, W_i = 1 \mid \X_i)}{\mbox{Pr}(W_i = 1 \mid Z_i = 1, \X_i)}.
\end{equation}
Because we only obtain measurements on firms who cheated and got caught, the data are only informative about $\Pr(Z_i=1, W_i=1\mid \X)$. Equivalently, for each firm-year we observe $Y_i \equiv Z_iW_i$ instead of $(Z_i, W_i)$, where $Y_i$ indicating whether a firm received an AER (cheated and got caught). Specifically, this is equivalent to the case described in Section \ref{sec:binreg}, with $U_1 = W$ and $U_2 = Z$.

%Note that $\mbox{Pr}(Y_i = 1 \mid \X_i)$ corresponds to the probability that a firm was issued an AAER in a given year, not the probability that its conduct warranted an AAER.  Again, many firms ``deserving" an AAER do not receive one; not all cheaters get caught.  To make this distinction explicit, we introduce two latent variables $Z_i$ and $W_i$ denoting ``cheating" and ``getting caught", respectively. Interest is in estimating the overall prevalence of accounting misconduct in the U.S. economy (between 2004 and 2012), which we define as 
%\begin{equation}
%\alpha = \displaystyle \sum_i \mbox{Pr}(Z_i=1 \mid \X_i) = \displaystyle\sum_i \frac{\mbox{Pr}(Z_i=1, W_i = 1 \mid \X_i)}{\mbox{Pr}(W_i = 1 \mid Z_i = 1, \X_i)}.
%\end{equation}
To cast this in the framework described in Section \ref{Kadane}, denote 
\begin{equation}
\phi(\X) = \mbox{Pr}(Z=1, W = 1 \mid \X) = \mbox{Pr}(Y  = 1 \mid \X); \;\;\; \theta(\X)  = \mbox{Pr}(W = 1 \mid Z = 1, \X).
\end{equation} 
%
Here $\phi(x)$ is simply the distribution of the observed data, and is point identified.  We estimate it using the BART model with default priors, except we set $k=3$.  This choice shrinks $\phi(\X)$ more strongly away from zero or one, which is particularly important in regions of predictor space with very few observations. In particular, it is unrealistic to expect that any company is {\em certain} to both cheat and get caught. The remaining parameter $\theta(x)$ is not identified and an informative prior must be supplied.  

\subsection{Simulated example}\label{sec:ex}
Before turning to the subject-specific prior we developed for our empirical application, it is instructive to consider how our approach performs in a situation where we know what the right answers ought to be. For this purpose we have design a simulated data set emulating the model in \cite{Wang2013}. This will be useful later when comparing our results to those in \cite{Wang2013} on the SEC data.

\subsubsection{A partially observed bivariate probit model}
Inspired by the approach of \cite{Poirier1980}, \cite{Wang2013} proposes a bivariate probit model for the $(W, Z)$ pairs described above.  In this formulation 


\subsection{Surveillance model}
The unidentified function $\theta(\X)$ can be thought of as a ``surveillance" probability; it encodes which attributes invite (discourage) SEC scrutiny, making cheaters more (less) likely to be caught.  Its effect is to inflate the probability of cheating, which is intuitive since the proportion of caught cheaters $\phi(x)$ represents an obvious lower bound on the proportion of actual cheaters.

Our surveillance model takes the form reported in expression (\ref{eq:theta-2}) with  $\epsilon_i \iid \N(0, \sigma^2)$ and using a logit link.  
Some care is required when specifying $h(\X)$. 
%We now describe the specification of $h(\X)$.  
Although BART is invariant to monotone transformations, the linear form of the surveillance model is not so it becomes important to choose transformations of the covariates so that the impact of firm features is plausibly scaled and we can specify reasonable values of $\beta$.  We therefore scale and shift all variables to reside on the unit interval, taking shifted log transformations of the financial times search hits and net income.
%To achieve this, we first  transform selected variables and then we scale and shift all variables to reside on the unit interval.  For our data, only two variables are transformed:  the financial times search hits variable and net income are both log transformed (after adding 1 to avoid taking the logarithm of zero).
%
%Setting the vector of regression coefficients, $\beta$, is where subject matter knowledge can be brought to bear.  Specifically, it allows us to surmise the impact of firm attributes on the probability of getting caught.  
%
We chose to place nonzero coefficients on the (fiscal) year of misconduct, media exposure (as measured by Financial Times search hits), income, cash, and a dummy for qui tam industries. We have specific reasons to expect that these variables are important determinants of the surveillance probability, allowing us to chose informative values for $\beta$.

First, note that the frequency of AAERs is substantially higher in earlier years; see Figure \ref{aaers}. AAERs may be filed retroactively, so the opportunity to discover and report misconduct in a given year increases over time.
%This is likely a simple byproduct of the fact that older cases of misconduct have had a longer time in which to be uncovered.  
%This suggests a negative coefficient on the fiscal year variable, meaning that more recent years are less likely to be spotted (yet).  
Fitting a curve to the data in Figure \ref{aaers} suggests a coefficient $\beta_{fyear} = -2.5$.  Observe that this makes the posterior probability of cheating approximately constant across the years examined, which seems plausible.
\begin{figure}
\begin{center}
\includegraphics[width=3in]{sec-figure/aaer_rate.pdf}
\end{center}
\caption{AAERs appear more common in more distant years, but this is likely because they may be filed retroactively.}\label{aaers}
\end{figure}

Second, it is reasonable to assume that media attention naturally draws SEC scrutiny \citep{miller2006press}.  
%Media darlings such as Apple, Amazon, and Google may be closely monitored because the SEC has a vested interest in making examples of such prominent businesses, should they misbehave.  
The SEC has a vested interest in catching and making examples of any high-profile cheaters.
We set $\beta_{FThits}=2$, implying approximately a six-fold difference in the probability of misconduct being discovered between a company with no media exposure and the company with the highest media exposure. Similarly, we set $\beta_{quitam}=1$, implying approximately a two-fold increase in misconduct being discovered for companies in qui tam industries where employees are incentivized to report misconduct.

These observations constitute the subjective information contained in our first observation model (A).  
To determine the intercept term, consider the following argument: AAERs are quite rare, with an aggregate incidence in our sample of only 0.5\%.  Potentially this is because very few firms exhibit actionable misconduct, but more likely it is because the SEC has limited resources to identify and pursue violations.  Accordingly, one sensible calibration method would be fix the mean probability of discovery across all firms.  Fixing this quantity and the other elements of $\beta$, we may then solve for the intercept $\beta_0$. In the case of model A, fixing the average discovery rate to 30\% gives $\beta_0 = 0$.

After obtaining posterior samples under model A, we observe that cash appears to have a negative impact on the probability of cheating. In contrast, net income appears to have a positive impact on the probability of cheating. We might surmise that these trends are due to unadjusted surveillance probabilities.  For example, one could argue that having large amounts of cash on hand (relative to total assets) provides a measure of ``wiggle room" that makes certain kinds of misconduct harder to discover.  Likewise, firms with high income are more likely to draw SEC attention than firms with smaller income streams.  To compare our results under these narratives, we specify a second surveillance model (B), with $\beta_{cash} = -1.5$ and $\beta_{income} = 2.5$.  Setting the intercept for model B to match the 30\% discovery rate of model A gives $\beta_0 = -0.85$.  Surveillance models  A and B are shown side-by-side in Table \ref{surveillance}.

\begin{table}
\begin{center}
\begin{tabular}{c|cccccc}
&Intercept&Fiscal year &FT.com hits&cash&net income&qui tam\\
\hline 
$\beta_A$ & $\;\;\;0$& $-2.5$&$2$&$0$& $0$& $1$\\ 
$\beta_B$ &$-0.85$&$-2.5$& $2$&$-1.50$&$2.5$&$ 1$\\
\end{tabular}\caption{Regression coefficients defining surveillance models A and B.  They differ in their intercept terms and their cash and net income coefficients.  The intercepts have been adjusted to obtain an average misconduct discovery rate of 30\%}\label{surveillance}
%the media-visibility proxy FT.com hits.  The intercepts have been adjusted to match the overall average probability of being caught, at 30\%.}
\end{center}
\end{table}

\subsubsection{Upper bounding cheating}\label{cparm}
Finally, we introduce an additional parameter $c$ to enforce a stochastic upper bound on the probability of cheating.  Recall that the partial identification in this application is driven by the inequality $\mbox{Pr}(Z = 1 \mid \X) = \frac{\phi(\X)}{\theta(\X)} \leq 1$, which implies $\phi(\X) \leq \theta(\X)$; the left hand side of this latter inequality is identified by the data.  
%If we are willing to stipulate that for any covariate values $\X$ a firm's probability of cheating is strictly less than one, this inequality instead becomes 
Extremely high probabilities of cheating are implausible, motivating us to consider alternative truncations: $\mbox{Pr}(Z = 1 \mid \X) = \frac{\phi(\X)}{\theta(\X)} \leq c$, which implies $\phi(\X)/c \leq \theta(\X)$ for $c \geq \phi(\X)$.  Because $\phi(\X)$ is identified, the data may contradict any particular value of $c$ by violating $c \geq \phi(\X)$ so $c$ is itself partially identified.  We continue our modular prior approach, placing a $\mbox{Beta}\left(10 c_0, 10(1-c_0)\right)$ prior on $c$, which {\em a posteriori} is sampled to obey the truncation implied by $\phi(\X)$.  Intuitively, the prior mean $c_0$ captures prior beliefs about the upper bound on $\mbox{Pr}(Z = 1 \mid \X)$, the probability of cheating for any firm.  

Our surveillance models allow us to include prior information in the form of
%As constructed, our surveillance models allow not only 
subject matter knowledge about the impact of various covariates. %to be incorporated, but also permit
We are also able to include additional subjective prior information about $\sum_i \mbox{Pr}(W_i = 1 \mid Z_i = 1, \X_i)$ --- the overall average probability of a cheating firm getting caught --- via the intercept terms, and $\mbox{max}_i \mbox{Pr}(Z_i = 1 \mid \X_i)$ --- an upper probability on any firm cheating --- via the prior on $c$. It would be difficult to acheive all these simultaneously without using the modular prior approach, which also facilitated the sensitivity analysis described below and a number of other iterations over candidate surveillance models that we do not have space to describe here.



\subsection{Results}
We conduct a sensitivity analysis by varying the parameters $\sigma$ and $c$ for both model coefficients $\beta_A$ and $\beta_B$ above.  Specifically, we consider two settings of each ($\sigma \in \lbrace 0.25,0.5 \rbrace$ and $c \in \lbrace 0.4,0.8 \rbrace$) for a total of eight candidate models.  We study the impact these choices have on both $\mbox{Pr}(Z=1 \mid \X)$ as a function of individual predictor variables, and also on the overall misconduct prevalence $\alpha$.

Figure \ref{SICboxplot} shows the posterior distribution of the adjusted cheating prevalence under the different models. As can be seen in the left-hand panel, increasing $\sigma$ or $c$ alone has little effect on the overall adjusted cheating prevalence. These two parameters control different aspects of the surveillance uncertainty: a high $c$ implies that any probability of cheating is plausible, whereas a high $\sigma$ allows large deviations from the specified surveillance model logistic term.  Note that with the range of $c$ and $\sigma$ chosen, neither surveillance model yields overall prevalence of misconduct greater than 15\%.

The right-hand panel of Figure \ref{SICboxplot} shows the posterior prevalence for each different SIC code under the two priors, fixing $(\sigma=0.25, c = 0.4)$. Under both priors, SIC category D, representing ``electricity, gas, steam and air conditioning supply'', shows much lower cheating prevalence than categories (B,E,H), which correspond to ``mining and quarrying'', ``water supply, sewerage, waste management and remediation activities'', and ``transportation and storage'' respectively. 
\begin{figure}
\begin{center}
\includegraphics[width=\textwidth]{sec-figure/boxplots.pdf}\\
\includegraphics[width=\textwidth]{sec-figure/SICboxplot.pdf}
\end{center}
\caption{Top panel: posterior cheating prevalence, white corresponding to the raw (unadjusted) prevalence, pink to prior A and blue to prior B. The four boxplots within each prior correspond to the following combinations for $c$ and $\sigma$ (from left to right): $(\sigma=0.25,c = 0.4),\;(\sigma=0.25, c = 0.8 ),\;(\sigma=0.5, c=0.4),\;(\sigma=0.5, c= 0.8)$. Bottom panel: Posterior cheating prevalence in companies within each SIC code, pink corresponding to prior A and blue to prior B for $(\sigma=0.25,c=0.4)$.  }\label{SICboxplot}
\end{figure}

Because BART is nonlinear, summary plots of the impact of individual covariates are challenging to visualize, even if the surveillance model is relative simple, such as our linear logistic specification.  It is instructive, therefore, to examine the implied probability of cheating as one varies individual covariates, for a given firm.  That is, how does $\mbox{Pr}(Z=1 \mid \X)$ change as a function of $x_j$ while holding $x_{-j}$ fixed?

To demonstrate this approach, we focus on a specific firm, ConAgra Foods of Omaha, Nebraska (simply because it yields illustrative plots).  Figure \ref{VaryPriorVarySC} shows $\mbox{Pr}(Z=1 \mid \X)$, varying media attention, cash, and net income under priors A and B and for various combinations of $c$ and $\sigma$. As expected, the surveillance model coefficients on cash and net income reverse the associated slope of the probability of cheating.  High values of both $\sigma$ and $c$ results in posterior credible intervals of up to 40\% probability of cheating for some values of net income. 

We have reported here only a small number of the possible variations one would presumably want to investigate; we make no claims that models A and B are ideal or even necessarily good or realistic models.  Rather, our sensitivity analysis demonstrates a range of possible comparisons that one might undertake when investigating how various assumptions interact with the data via the identified portion of the model.  

An important upshot of our analysis is that the surveillance model intercept terms---which govern the  average probability of misconduct discovery (getting caught) across firm---and the parameter $c$--- which defines the upper bound $\mbox{Pr}(Z_i =1 \mid \X_i) \leq c$ for all $i$ --- play dominant roles in determining the inferred overall prevalence of misconduct.  For our choices of 30\% misconduct discovery probability and $c = 0.4$ or $c=0.8$, we find that no more than 15\% of firms engage in accounting misconduct.  


\begin{figure}
\begin{center}
\includegraphics{sec-figure/priorAB.pdf}
\end{center}
\caption{$\mbox{Pr}(Z=1 \mid \X)$ varying $x_j$ while holding $x_{-j}$ fixed (at the values of ConAgra Foods) under two surveillance models A (pink) and B (blue). Lines depict the median and shaded areas depict 90\% credibility intervals. Each row represents a different covariate; the three columns correspond to the following $(c, \sigma)$ combinations (from left to right): $(c=0.4,\sigma=0.25),\;(c=0.8,\sigma=0.25),\;(c=0.8,\sigma=0.5)$. }\label{VaryPriorVarySC}
\end{figure}

==> fig/fig.tex <==



\begin{figure}
\begin{center}
\begin{tikzpicture}[
  scale=1.1,
    node/.style={%
      draw,
      rectangle,
    },
    node2/.style={%
      draw,
      circle,
    },
  ]

    \node [node] (A) {$x_1<0.8$};
    \path (A) ++(-135:\nodeDist) node [node2] (B) {$\mu_{h1}$};
    \path (A) ++(-45:\nodeDist) node [node] (C) {$x_2<0.4$};
    \path (C) ++(-135:\nodeDist) node [node2] (D) {$\mu_{h2}$};
    \path (C) ++(-45:\nodeDist) node [node2] (E) {$\mu_{h3}$};

    \draw (A) -- (B) node [left,pos=0.25] {no}(A);
    \draw (A) -- (C) node [right,pos=0.25] {yes}(A);
    \draw (C) -- (D) node [left,pos=0.25] {no}(A);
    \draw (C) -- (E) node [right,pos=0.25] {yes}(A);
\end{tikzpicture}
%
\hspace{0.1\linewidth}
\begin{tikzpicture}[scale=4]
\draw [thick, -] (0,1) -- (0,0) -- (1,0) -- (1,1)--(0,1);
\draw [thin, -] (0.8, 1) -- (0.8, 0);
\draw [thin, -] (0.0, 0.4) -- (0.8, 0.4);
\node at (-0.1,0.4) {0.4};
\node at (0.8,-0.1) {0.8};
\node at (0.5,-0.2) {$x_1$};
\node at (-0.3,0.5) {$x_2$};
\node at (0.9,0.5) {$\mu_{h1}$};
\node at (0.4,0.7) {$\mu_{h2}$};
\node at (0.4,0.2) {$\mu_{h3}$};
\end{tikzpicture}
\end{center}
\caption{(Left) An example binary tree, with internal nodes labelled by their splitting rules and terminal nodes labelled with the corresponding parameters $\mu_{hb}$ (Right) The corresponding partition of the sample space and the step function.}
\label{fig:treestep}
\end{figure}



==> flu_ArXiV.tex <==
%!TEX root = HahnMurrayManolopoulou_ArXiV.tex

Our data come from a randomized encouragement study of the effectiveness of an influenza vaccine conducted at an academic primary care practice affiliated with a large teaching hospital in an urban setting \citep{McDonald1992}. Physicians were randomly assigned to treatment or control groups, with treated physicians receiving a computerized reminder about the vaccine when a patient with a scheduled visit also met the U.S. Public Health Service Criteria for receiving a flu vaccine. Patients were eligible for the vaccine if they were 65 or older, or if they had certain severe chronic diseases including chronic obstructive pulmonary disease (COPD).
% lung disease, asthma, diabetes, congestive heart failure, or severe liver or kidney failure. 
The outcome of interest is subsequent hospitalization for flu-related illness, and the covariates include the patient's age and COPD status. \cite{Hirano2000} conduct a Bayesian analysis of this problem, placing a default joint prior over all the identified and unidentified parameters. In this application we perform an alternative selectively informative analysis with modular priors. %One aspect of this design which has been ignored to date is that the inclusion criteria potentially induce a sharp change in the probability of a positive outcome at age 65, since anyone 65 or older was in the study population while a 64 year-old patient would only be included if he or she had a serious, chronic disease.
We will use the terms ``reminder'', ``instrument'' and ``encouragement'' interchangably here, prefering ``reminder'' in the context of the specific applied problem.
 
\subsection{Causal Inference in a Binary Instrumental Variables Model}
%\sayan{fix to make everything conditional on X (doesn't change anything substantively)} 

Let $Z_i, T_i$, and $Y_i$ be the observed values of the treatment assignment (or encouragement, or instrument), treatment received, and outcome for observation $i$, respectively.  Let $X_i$ be a vector of baseline covariates. In the flu data, $Z_i=1$ if encouragement (the reminder) was administered, $T_i=1$ if the vaccine was administered, and $Y_i=1$ if the patient was \emph{not} hospitalized. As in \cite{Angrist1996} and \cite{Hirano2000} define the \emph{potential outcomes} $T_i(z)$ and $ Y_i(t,z)$ as the treatment
assignment that would have been observed had we fixed $Z_i=z$ and the outcome we would have observed fixing $T_i=t, Z_i=z$, respectively. We will suppress indexing by $i$ for population quantities. We make the stable unit treatment value assumption (SUTVA) \citep{Angrist1996}, i.e. that there is no interference between units and no alternative versions of treatment. \footnote{\cite{Hirano2000} point out that in an infectious disease application with individuals as the unit of randomization this assumption is unlikely to hold exactly, but constitutes a reasonable first order approximation.} Mathematically, SUTVA implies that $T_i(\mathbf{z})=T_i(z_i)$ and $Y_i(\mathbf{t}, \mathbf{z})=Y_i(t_i, z_i)$, where $\mathbf{z}, \mathbf{t}$ are vectors of instrument/encouragement assignment and treatments received (respectively) for the entire sample.

In this application the complete vector of binary response variables is 
\begin{equation}
U_i=(T_i(0), T_i(1), Y_i(0,0), Y_i(0,1), Y_i(1,0), Y_i(1,1))',
\end{equation}
 the collection of treatments and outcomes under all possible experimental conditions. However, we observe only $T_i\equiv T_i(Z_i)$ and $Y_i\equiv Y_i(T_i(Z_i), Z_i)$, where $Z_i$ is randomly assigned at the study outset. 
%
%as follows:
%\begin{equation}
%T_i = Z_iT_i(1) + (1-Z_i)T_i(0)
%\end{equation}
%\begin{equation}
% Y_i = T_iZ_iY_i(1,1) + 
%(1-T_i)Z_iY_i(0,1) + 
%T_i(1-Z_i)Y_i(1,0) + 
%(1-T_i)(1-Z_i)Y_i(0,0).
%\end{equation}
%
We can define compliance types or principal strata $S$ based on the possible values for $(T(1), T(0))$ -- see Table \ref{tab:comptype}. 
%
\begin{table}
\begin{center}
    \begin{tabular}{cc|ll}
        $T(1)$ & $T(0)$ & $S$ (Compliance Type) & ~    \\ \hline
        0     & 0     & Never Taker     & (n) \\ 
        1     & 1     & Always Taker    & (a) \\ 
        1     & 0     & Complier        & (c) \\ 
        0     & 1     & Defier          & (d) \\
    \end{tabular}
  \caption{Compliance types, or principal strata, defined by response patterns across levels of $Z$.}
  \label{tab:comptype}
  \end{center}
\end{table}
%
We will assume that the encouragement $Z$ is ignorable or randomly assigned (as it is in the flu data).
We also assume that there are no defiers (``monotonicity of compliance"), i.e., $ \Pr(S=d\mid \X)=0$. In the current setting a defier would be a patient who would \emph{only} receive the vaccine if the reminder was \emph{not} administered, which is quite unlikely.

Let $\pi_s(x) = \Pr(S=s\mid \X)$  and 
$\gamma^{tz}_s(x) = \Pr( Y(t,z)=1\mid S=s, \X)$ denote the principal strata and potential outcome probability models. Under the above assumptions the potential outcome and principal strata distributions are linked to the joint distribution of observables by the following equations.
%
\begin{align}
\Pr(T=1\mid Z=0, \X) &= \pi_a(\X)\label{eq:mon-1},\\
\Pr(T=1\mid Z=1, \X) &= \pi_c(\X) + \pi_a(\X)\label{eq:mon-2},\\
\Pr(Y=1\mid T=0, Z=0, \X) &= [\pi_c(\X)\gamma^{00}_c(\X) + \pi_n(\X)\gamma^{00}_n(\X)]/[\pi_c(\X) + \pi_n(\X)]\label{eq:mon-3},\\
\Pr(Y=1\mid T=1, Z=1, \X) &= [\pi_c(\X)\gamma^{11}_c(\X) + \pi_a(\X)\gamma^{11}_a(\X)]/[\pi_c(\X) + \pi_a(\X)]\label{eq:mon-4},\\
\Pr(Y=1\mid T=0, Z=1, \X) &= \gamma^{01}_n(\X),\\
\Pr(Y=1\mid T=1, Z=0, \X) &= \gamma^{10}_a(\X)\label{eq:mon-last}.
\end{align}
\cite{Richardson2010} derive this mixture relationship between principal strata/potential outcome distributions and the observable joint in detail under a range of assumptions about the latent variables (see also \cite{Imbens1997a} and \cite{Richardson2011}).

The probabilities on the left hand side completely determine the joint distribution of observables ($Y$ and $T$ given $Z$) and hence constitute a basis for $\phi$. Clearly $\pi$, $\gamma^{01}_n$ and $\gamma^{10}_a$ are one-to-one maps from $\phi$, and are point identified as well. However, $\gamma^{00}_c,\ \gamma^{00}_n,\ \gamma^{11}_c,$ and $ \gamma^{11}_a$ are not. For example, at any point in covariate space $\gamma^{11}_c(x)$ and $\gamma^{11}_a(x)$ must lie on the line segment given by the intersection of the line in equation \eqref{eq:mon-4} and $[0,1]\times [0,1]$, but the data are wholly uninformative about their position on that line segment. In particular, the range of $\gamma^{11}_a(x)$ is

\begin{equation}
\left(
	\min\left(
		0, \frac{\pi_a(x)+\pi_c(x)}{\pi_a(x)}p_{1\mid 11}(x) - \frac{\pi_c(x)}{\pi_a(x)}
	\right),\,
	\max\left(
		1, \frac{\pi_a(x)+\pi_c(x)}{\pi_a(x)}p_{1\mid 11}(x)
	\right)
\right)\label{eq:gbound}
\end{equation}
where $p_{1\mid 11}(x) = \Pr(Y=1\mid T=1, Z=1,\X)$. The situation is exactly the same for $\gamma^{00}_c(x)$ and $\gamma^{00}_n(x)$, with the line given by \eqref{eq:mon-3} and bounds similar to \eqref{eq:gbound} (large sample bounds on causal effects within principal strata were introduced by  \cite{zhang2003estimation}; see \cite{Richardson2011} for bounds under monotonicity and other assumptions, as well as further references).

%j 7/29
%In the instrumental variables literature, 
Point identification for the remaining parameters is often obtained through further assumptions on the distribution of the potential outcomes. The \emph{stochastic exclusion restriction} for compliance type $s$ posits that there is no direct effect of $Z$ on $Y$; that is, $\gamma^{i0}_s = \gamma^{i1}_s$ for $i=0,1$ \citep{Hirano2000}. From \eqref{eq:mon-1}-\eqref{eq:mon-last} it is clear that this achieves point identification for the entire distribution of the potential outcomes.

\cite{Hirano2000} anticipated failures of the exclusion restrictions, noting that a reminder about flu shots might also prompt physicians to counsel patients about other preventative measures to avoid contracting the flu. They propose relaxing the exclusion restrictions and resolving the resulting nonidentifiability through prior probability modeling. In this sense our approach and theirs are philosophically similar, but our framework affords us significant flexibility in choosing the model for $\phi$ while transparently embedding prior information about $\theta$, which is difficult to do in their modeling setup. In our subsequent analysis we will avoid imposing any exclusion restrictions.
%
% What will be particularly relevant for our  analysis is that any direct effect of the reminder on subsequent hospitalization for flu-related illness should be positive and relatively small, and is likely to be larger in always takers than in never takers (since one factor driving uptake of the vaccine and other prophylactic measures is perceived risk, which is higher in always takers).
%
%
%
%
%
%Our focus will be on \emph{intention-to-treat (ITT)} effects. The sample ITT effect is 
%
%\begin{equation}
%ITT = \frac{1}{n}\sum_{i=1}^n (Y_i(T_i(1), 1) - Y_i(T_i(0), 0)). 
%\end{equation}
%Sample ITT effects for different compliance types are defined similarly:
%\begin{equation}
%ITT_s = \frac{1}{n_s}\sum_{i: S_i=s} (Y_i(T_i(1), 1) - Y_i(T_i(0), 0)). 
%\end{equation}
%where $n_s$ is the number of observations with compliance type $S$ \citep{Hirano2000}. 
%The potential outcome distributions $\gamma$ and compliance type distributions $\pi$ are linked to the joint distribution of observables by the following equations (suppressing the dependence on $x$):
%
%\begin{align}
%\Pr(T=1\mid Z=0) &= \pi_D + \pi_a\\
%\Pr(T=1\mid Z=1) &= \pi_c + \pi_a\\
%\Pr(Y=1\mid T=0, Z=0) &= (\pi_c\gamma^{00}_c + \pi_n\gamma^{00}_n)/(\pi_c + \pi_n)\\
%\Pr(Y=1\mid T=1, Z=1) &= (\pi_c\gamma^{11}_c + \pi_a\gamma^{11}_a)/(\pi_c + \pi_a)\\
%\Pr(Y=1\mid T=0, Z=1) &= (\pi_D\gamma^{01}_D + \pi_n\gamma^{01}_n)/(\pi_D + \pi_n)\\
%\Pr(Y=1\mid T=1, Z=0) &= (\pi_D\gamma^{10}_D + \pi_a\gamma^{10}_a)/(\pi_D + \pi_a).
%\end{align}
%
% Assuming the exclusion restriction in always and never takers point identifies the (population) intent to treat effect in compliers:
%\begin{equation}
%PITT_{C} = \gamma^{11}_c - \gamma^{00}_c,
%\end{equation}
%which is equivalent to the local average treatment effect (LATE) if the exclusion restriction holds in compliers as well \cite{Angrist1996}. In the absence of the exclusion restrictions for always takers and/or compliers, $PITT_c$ is bounded by the equations above and the fact that the $\gamma$'s are probabilities. Since the data are informative about these bounds (the bounds themselves are point identified) $PITT_c$ is \emph{partially} identified.
%
%There are theoretical and empirical reasons to suspect that the exclusion restrictions might be violated. \cite{Richardson2011} give a detailed exposition of bounds on the joint distribution of $(Y, T\mid Z)$ induced by assuming various combinations of monotonicity and the exclusion restrictions.  \cite{Richardson2011} compute posterior distributions of these bounds under a Dirichlet-multinomial model without covariates. Assuming monotonicity, they find that the posterior probability of violating the bounds is 0.54 and 0.06 for the exclusion restriction in always takers and never takers respectively. Since the bounds are necessary but not sufficient for the exclusion restrictions to hold, there is ample evidence that the exclusion restrictions are violated.

\subsection{Model Specification}

Our model for observables decomposes into a treatment model and an outcome given treatment model, i.e., $P(Y,T\mid Z, \X) = P(T\mid Z, \X)P(Y \mid T, Z, \X)$. We assign each of these a probit BART prior. For the treatment model, randomization of treatment assignment and monotonicity of compliance imply that $\Pr(T=1\mid Z=1, \X) \geq \Pr(T=1\mid Z=0, \X)$ for all $\X$ (see equations \eqref{eq:mon-1} and \eqref{eq:mon-2}). We enforce this constraint by rejecting samples from BART where this condition fails at any point in covariate space. More elaborate approaches to enforcing monotonicity are possible but beyond the scope of the present paper. %As we are not imposing any exclusion restrictions, there are no constraints on our model for the outcome given the treatment and instrument. 

\subsubsection{Partially identified parameters}

Recall that we have two pairs of unidentified parameters,  $(\gamma^{00}_c, \gamma^{00}_n)$ and $(\gamma^{11}_c,\gamma^{11}_a)$. Fixing one element of each pair would solve the identification problem, so we can take $\theta = (\gamma^{00}_n,\gamma^{11}_a)$ without loss of generality. 
%Other parameterizations of $\theta$ are of course possible, but this choice will be convenient for prior specification. 
This is in contrast to \cite{Hirano2000}, who specify a strongly parametric probability model for all four of the unidentified parameters.

We consider three priors on $\theta$. All three are of the form
\begin{equation}
(\mbox{logit}\{\gamma^{00}_n(\X)\}, \mbox{logit}\{\gamma^{11}_a(\X)\})' = \mu\{\phi(\X)\} + h(\X)\beta + \epsilon(x)\label{eq:theta-3}.
\end{equation}
with $\mu(\phi(\X)) = (\mbox{logit}\{\gamma^{01}_n(\X)\}, \mbox{logit}\{\gamma^{10}_a(\X)\})'$, $h(\X)=1$ and $\beta=(b_a, -b_n)$. This centers our prior at a proportional odds model, where the reminder increases the odds of a positive outcome by a factor of $\exp(b_a)$ or $\exp(b_n)$ in always or never takers (respectively) at any covariate value. A natural way to complete this prior is to take $b_s\sim N(0, \sigma_s^2)$ for $s=a,n$ which centers the prior at the exclusion restrictions and expresses prior beliefs about plausible effect sizes through $\sigma_s^2$. For illustration we take $\sigma_s=0.1$ or $0.25$ for the current application. \cite{Hirano2000} estimate principal strata-independent total effects of COPD around -0.35 on the log odds scale, so the more diffuse prior covers a plausible range of possible effect sizes for the direct effect of a reminder within non-compliers.  We would expect any direct beneficial effect of the reminder on the subsequent hospitalization to be smaller than the detrimental effect of a serious chronic disease like COPD purely on substantive grounds.

In the flu application we also have some prior information about likely effect directions, which we can also incorporate in the prior. 
%As observed by \cite{Hirano2000}, 
Any direct effect from the reminder is most likely to be positive, since the reminder probably encourages doctors and patients to take other preventative measures beyond the vaccine. Additionally, \cite{Hirano2000} speculate that the exclusion restriction for never takers is more plausible than for always takers since perceived risk is a key driver of compliance behavior, with low-risk patients more likely to be never takers. A more nuanced view is that the direct effect should be \emph{larger} for always takers than never takers --- even though never takers probably have lower risk on average, we should not rule out the possibility of high-risk never takers who refuse the vaccine due to cost, safety or other concerns. 

A prior for $\theta$ that reflects these beliefs is $(b_a, b_n)\sim \N(b_0, \Sigma_b)\mathbb{1}(b_a>0, b_n>0)$. For the analysis in the sequel we will take $b_0 = (0.05, 0.0)'$, $\Sigma_b = \mbox{diag}(0.13^2, 0.05^2)$. In additional simulations we find that results are insensitive to plausible values of $\mbox{Cov}(b_a, b_n)$. These particular numerical values were chosen  The prior mode is $b_0$, the prior mean is about $(0.125, 0.04)$, and the marginal $90^{th}$ percentile is about 0.25 for $b_a$ and 0.08 for $b_n$. 
%This prior is calibrated so that the direct effect in any takers is larger than that for never takers and both are positive. 
The prior scale for $b_a$ is calibrated so that (with high probability) $b_a$ is smaller in magnitude than the effect of COPD on the hospitalization as reported by \cite{Hirano2000} (the posterior mean was generally around -0.35, SD 0.15). We will call this the ``informed" prior.
For all three priors we set $v=0.025$. 
%$v(x)$ as 
%\begin{equation}
%v(x, \phi) = \{0.025[1 + 200\delta_{x}]\}^2
%\end{equation}
%where 
%$
%\delta_{x} =
%  %\begin{cases}
%   %0 & \text{if } a(\phi(x)) < m(\X^*_j) < b(\phi(x))) \\
%   \max\{0, a(\phi(x))-m(x),\ m(x)-b(\phi(x))\}      %& \text{otherwise}  \end{cases}
%$.

%Even leaving aside this additional information, it is hard to imagine the hypothesized mechanisms for the direct effect  having effects larger than 25 or 30\%, so this prior seems  reasonable.

%
%We describe prior specification for $\gamma^{11}_a(x)$ since the prior on $\gamma^{00}_n(x)$ will be specified similarly. Let $\eta_a^{11}(x)=\logit(\gamma^{11}_a(x))$. We induce a prior on $\gamma_a^{11}$ by assuming a Gaussian process prior on $\eta_a^{11}$:
%\begin{equation}
%\left(\eta_a^{11}(x_1), \eta_a^{11}(x_2),\dots,\eta_a^{11}(x_q)\right)'\sim N((m_{A}(x_1), m_{A}(x_2),\dots,m_{A}(x_q))', \tau_a\Sigma_a(x_1, x_2,\dots,x_q))
%\end{equation}
%
%for some mean function $m$ and covariance function $\Sigma$, where $x_1,x_2,\dots x_q$ are design points of interest. For inference on sample average treatment effects these should be the distinct covariate values observed in the dataset. The scale parameter $\tau_a$ expresses our overall confidence in the specification of the mean function and could also vary with $x$ if appropriate. Since we are primarily interested in $ITT_c$, an additive function of $\gamma^{11}_a(x)$ and $\gamma^{00}_n(x)$, there is little benefit to enforcing smoothness in $\gamma^{11}_a$ or $\gamma^{00}_n(x)$ so we simply take $\Sigma(x_1, x_2,\dots,x_q) = \tau_a^2I$. 
%
%Any number of mean functions are possible. One natural choice is 
%
%\begin{equation}
%m_a(x) = a_a + \logit(\gamma^{10}_a(x)),\label{eq:propoddsA}
%\end{equation}
%
%which centers our prior on a constant proportional odds model (the reminder increases the odds by a multiplicitive factor of $e^{\alpha_a}$ at any covariate value). The value of $\alpha_a$ can be varied over a range of plausible values, or given an informative prior itself. The conditional prior on $m_n$ will be similar:
%\begin{equation}
%m_n(x) = -a_n + \logit(\gamma^{01}_n(x)),\label{eq:propoddsN}
%\end{equation}
%where the negative intercept is to keep $\alpha_a$ and $\alpha_n$ consistent in sign (positive values indicating a protective effect of the reminder).
%
\subsection{Results}

We fit the model described in the previous section to the flu vaccine data, using age and COPD as covariates. Figure \ref{fig:psmembership} shows the probability of belonging to each principal stratum as a function of age and COPD along with marginal 90\% credible intervals. We find a fairly sharp break in compliance behavior at age 65 (the probability of being a never-taker drops, and seems to be shifted largely to always takers), which appears to hold regardless of COPD status. Possible explanations include patients or providers giving more weight to age-based vaccination guidelines, or better insurance coverage and increased access to services in the older cohort. 

Figure \ref{fig:outcometz} shows the outcome distributions by age, COPD, and the treatment assigned and received. There is clear evidence of an age/COPD interaction; this is due at least in part to the study design, where all participants under 65 have at least one chronic disease (possibly COPD). This also means that the 65+ population is on average less likely to he hospitalized than the younger cohort, explaining the seemingly paradoxical decrease in the estimated probability of hospitalization at age 65 in the ``No COPD" group.

\begin{figure}
\begin{center}
\includegraphics[width=5in]{flu-figure/PSMembershipTrunc.pdf}
\caption{Principal strata memberhsip probabilities by age and COPD, including marginal 90\% credible intervals}\label{fig:psmembership}
\end{center}
\end{figure}

\begin{figure}
\begin{center}
\includegraphics[width=3.5in]{flu-figure/OutcomeByTZ.pdf}
\caption{Log odds of a positive outcome (no hospitalization) by age, COPD, and treatment assignment/receipt}\label{fig:outcometz}
\end{center}
\end{figure}


\subsubsection{Causal effects}
We are primarily interested in (partially identified) sample causal effects. 
%Recall that for each unit we observe $T_i(Z_i)$ and $Y_i(T_i(Z_i), Z_i)$, but individual level causal effects (and their averages) are defined in terms of contrasts between potential outcomes; for example, the individual \emph{intent to treat} (ITT) effect for unit $i$, the total effect of the instrument on the response, is $Y_i(T_i(1), 1) - Y_i(T_i(0), 0)$. 
As in \cite{Hirano2000} we will consider estimating the intention-to-treat (ITT) effect in each principal stratum:
\begin{equation}
ITT_s = \frac{1}{n_s}\sum_{i: S_i=s} (Y_i(T_i(1), 1) - Y_i(T_i(0), 0)). 
\end{equation}
where $n_s$ is the number of observations with compliance type $S$. Given a sample from the marginal distribution for $\phi$, and a sample from $\theta$, we can impute each observation's missing principal strata membership and the unobserved potential outcome. With the completed data it is straightforward to compute the sample ITT effects. Computational details are provided in Appendix \ref{app:postmis}

%We also fit the BART model using the full set of covariates in the flu data, which also include race, sex, and indicators for other chronic conditions (diabetes and heart, liver, and kidney disease). \cite{Hirano2000} choose baseline variables based on imbalance in the two $T$ arms, but any variable which predicts compliance behavior or hospitalization risk has the potential to tighten the bounds on $\theta$ (see \cite{Long2013} and the references therein for an asymptotic argument). Note that this is an argument for incorporating baseline covariates that predict the outcome \emph{or} have a significant interaction with $Z$ in the treatment model, rather than basing variable inclusion on balance with respect to $T$. 

%The treatment model is much more discriminative with the extra variables, and it turns out that this is due largely to race (Figure \ref{fig:flupc}). Significant differences in vaccine uptake among different racial/ethnic groups have been observed for some time, even after controlling for age and other risk factors ((cites)), so this result is somewhat unsurprising.
%
%\begin{figure}
%\begin{center}
%\includegraphics[width=4in]{flu-figure/flupc.pdf}
%\caption{Posterior mean estimates of $\pi_c(x)$ from the BART treatment model with age/COPD and the full set of covariates}
%\end{center}
%\label{fig:flupc} 
%\end{figure}

We compare results under our three priors to three models from \cite{Hirano2000}: the model with no exclusion restrictions (``none"), both exclusion restrictions (``both"), or the never-taker exclusion restriction (``n"). The ``Hirano (none)" model has very wide standard deviations, which are driven by their use of diffuse, ``off-the-shelf" priors.  Their marginal prior for the direct effect of the reminder is approximately normal with mean zero and standard deviation 1.5, which puts significant prior probability on implausible values such as large and/or negative direct effects. Such vague priors are inappropriate for partially identified parameters.

In contrast, the BART models all give similar results. The ``BART (0.1)" and ``BART (0.25)" models differ mainly in the width of the posterior standard errors, and then only slightly. The ``BART (0.25)" model assumes that with high probability the magnitude of any direct effect on the log odds is within $\pm 0.5$ -- compare this to the COPD effect, which is estimated to increase the log odds of hospitalization by about 0.35. The ``informed" prior restricts the population effects to be positive but small, which tends to shrink the $ITT_c$ effect toward zero -- the overall $ITT$ effect is identified, so positive effects in the other principal strata lead necessarily to smaller $ITT_c$ estimates than unrestricted models.

The substantive conclusion is largely unchanged: there is only modest evidence for the effectiveness of the vaccine, particularly if we assume the direct effect of the reminder is similar in always-takers and compliers. This is unsurprising given the sample size of $n=2,861$, weakness of the encouragement (Fig. \ref{fig:psmembership}), and relative rarity of the outcome (about 8\% of the study participants were hospitalized). However, unlike \cite{Hirano2000} we conclude that the $ITT_c$ effect is actually fairly robust to plausible deviations from the exclusion restrictions.

%In contrast, the standard deviation of the $ITT_c$ effect in the ``BART (age/COPD)" model is comparable to the point identified ``Hirano (both)" model, despite making no strong assumptions about the functional form of the observable joint distribution (unlike \cite{Hirano2000}) and allowing for deviations from the exclusion restrictions. The estimate of $ITT_c$ is apparently robust to reasonable deviations from the exclusion restrictions. The substantive conclusion from the age/COPD model changes little, however: Assuming the direct effect of the reminder is similar in always-takers and compliers, there is only modest evidence for the efficacy of the flu vaccine. The evidence from the all-covariate model is somewhat stronger in favor of the vaccine. The posterior mean effect is notably larger (0.114 vs 0.086), with a smaller standard deviation (0.064 vs 0.072) while the always- and never-taker effects change very little. 

\begin{figure}
\begin{center} 
\includegraphics[width=5.25in]{flu-figure/flures.pdf}
\caption{Posterior mean and standard deviations for the sample ITT effects in each principal stratum. ``BART (0.1)" and ``BART (0.25)" use the conditional prior centered at the exclusion restrictions with $\sigma_a=\sigma_n=0.1$ or $0.25$, respectively. ``BART (informed)" includes all prior information. The ``Hirano" models are from \cite{Hirano2000}; the ``n" model assumes the exclusion restriction in never-takers, the ``both" model imposes both exclusion restrictions and the ``none" model has no exclusion restrictions.}\label{fig:flures}  
\end{center}
\end{figure}


%Our prior is carefully constructed to represent scientifically plausible states of the world, unlike the ``off-the-shelf" prior proposed in \cite{Hirano2000}. Their marginal prior for the direct effects is approximately normal with a mean of zero and standard deviation 1.5, which puts significant prior probability on implausible values such as large, negative direct effects. These vague priors are not generally good practice in partially identified problems and are at least part of the reason why the authors find little evidence of a positive effect of the vaccine.

%why posterior variance go down bro?
 
%We could go further and let
%\begin{equation}
%m_a(x) = \alpha_a + x'\beta_a + \logit(\gamma^{10}_a(x)),
%\end{equation}
%perhaps fixing some subset of $\beta$ to be identically zero and either setting the rest at plausible values or assigning them prior distributions. Note that the linear term $x'\beta$ should be interpreted as an interaction between covariates and treatment assignment, since we have included $\logit(\gamma^{10}_a(x))$ in the mean function. 



==> sec.tex <==
%The goal of our analysis is not to provide a definitive estimate of the fraction of U.S. firms that misreport; indeed a precise estimate will vary depending on the assumptions one brings to the analysis.  Rather our goal is to provide a framework for permitting interested individuals to compare differing conclusions on a common basis, by systematically combining the same data with varying assumptions about the observation process.  To be sure, sensitivity analysis has long been advocated (\cite{Leamer1978}) although in our experience these appeals are more honored in the breach than in the observance.  Our present efforts are intended to make sensitivity analysis as straightforward as possible so that model fitting does not have to be undertaken anew each time an additional observation model is entertained.  Additionally, our approach is to use an exceptionally flexible nonlinear regression method to estimate the identified portion of the model; this is in contrast to the relatively common practice of choosing a model which resolves non-identification in a way that simultaneously restricts the identified portion of the model (perhaps inappropriately).  Examples of this phenomenon are provided in the literature review below.
 

Since 1982, the United States Securities and Exchange Commission (SEC) has released public notices called Accounting and Auditing Enforcement Releases, or AAERs.  AAERs are financial reports ``related to enforcement actions concerning civil lawsuits brought by the Commission in federal court and notices and orders concerning the institution and/or settlement of administrative proceedings"  \citep{SECwebsite}. Informally, AAERs comprise a list of publicly traded firms that the SEC has cited for misconduct in one form or another.  

For brevity, we adopt the nomenclature ``cheating'' and ``caught'', with the understanding that ``cheating" is operationally defined as any accounting anomaly that would lead to an AAER being issued, were it explicitly brought to the SEC's attention.  This interpretation entails that no ``caught" firms did not ``cheat", by definition.

Our goal is to provide an estimate of the prevalence of accounting misconduct in the U.S. economy, defined as all actual (caught) and potential (uncaught) AAERs.  Predicting which companies are likely to cheat, on the basis of observable firm characteristics, is complicated by the fact that there are potentially many instances of misconduct of which the SEC is unaware.  Thus, we do not directly observe which firms cheat, but merely the subset of cheating firms that were {\it caught} doing so.  A naive regression analysis would therefore only speak to the question of which attributes are predictive of getting caught cheating.  To complete the analysis, one must incorporate knowledge or conjectures concerning the impact firm attributes have on the likelihood of misconduct being discovered.  

Problems with similar structure appear in the literature under the heading of ``partially observed binary data".  Regression models for such data have been studied in many different fields, going by various names.  For example, \cite{Lancaster1996} considers the case where the observation model is covariate independent under the name ``contaminated case-control", building on \cite{prentice1979logistic}.  \cite{poirier1980partial} studies such data under the rubric of ``partially observed bivariate probit models", building on the work of \cite{Heckman1976,Heckman1978,Heckman1979}.  Our analysis follows closely the approach taken in \cite{Dyck2013}, where the prevalence of financial misreporting is tackled via several methods, including the bivariate probit model of \cite{poirier1980partial} which was suggested specifically for the securities fraud problem in \cite{Wang2013}.
 
Key references concerning the more general problem of likelihood-based inference in the presence of missing data and/or biased sampling include \cite{rubin1976inference,dawid1977likelihood, little1987statistical, efron1994missing} and \cite{chib2009estimation}, to name but a few.
 
\subsection{Data}
Our data are aggregated from three main sources.  First, the AAER response variable was obtained from the Center for Financial Reporting and Management (CFRM) at Berkeley's Haas School of Business.  Detailed information about the full data set can be found in \cite{dechow2011predicting}. 

Second, additional firm attributes are obtained from the CompuStat North America Annual Fundamentals database via the Wharton Research Data Service (WRDS).  These data are then merged with the AAERs using Global Company Key (GVKEY) by year.  Specifically, the features considered are:
\begin{itemize}\addtolength{\itemsep}{-0.5\baselineskip}
\item fiscal year,
\item cash,
\item net income,
\item capital investments,
\item SIC industry code,
\item qui tam dummy variable.
\end{itemize}
\noindent Cash, net income and capital investments are all recorded as a fraction of the firm's total assets.  Standard industrial classifications are given in terms of ten major divisions, denoted A-J by the Occupational Safety and Health Administration.  The {\em qui tam} dummy variable is derived from the SIC codes; it denotes if a firm is in an industry where persons responsible for revealing misconduct are eligible to receive some part of any award resulting from subsequent prosecution.  Similar to \cite{dyck2008corporate} and  \cite{jayaraman2010whistle}, our qui tam variable is set to one for firms with SIC code 381x, 283x, 37xx, 5122 or 80xx, which includes healthcare providers and pharmaceutical firms, and airplane, missile, and tank manufacturers.  It is reasonable to suppose that firms in these industries have a greater likelihood of any misconduct being exposed as a result of incentivized employees.  

Finally, a keyword search at the Financial Times web page (www.ft.com) was conducted on each company name and the number of search results was recorded by year.  This variable provides a crude measure of media exposure.  Although discrepancies between firm names as recorded in CompuStat and firm names as reported in Financial Times articles lead to measurement error of this variable, it still provides a  reasonable proxy for name recognition and cultural visibility. Most firms will never be mentioned in any news article; a few firms are routinely mentioned in the press. To adjust for the fact that web traffic has increased over that period, we normalize the search results count by the total number of hits across all companies in a given year.

We restrict our analysis to U.S. firms who had positive net income for the given year, considering the period between 2004 and 2010, for a total of $6,641$ unique firms and a total of $n=25,889$ total firm-year observations.

\subsection{Model specification}
%We index our firm-year observations by $i = 1, \dots, n$. 
Let $Z_i$ indicate ``cheating" in firm-year $i$ and let $W_i$ indicate ``getting caught" in firm-year $i$. We assume that with some probability cheaters get caught, but there are no firms who get caught when they are not cheating (this is consistent with our operational definition of ``cheating"). Additonally, the data is ``presence-only'' in that we have no confirmation that any given firm is for sure non-cheating.  We would like to infer $\Pr(Z_i\mid \X)$, which would allow us to compute an aggregate estimate of cheating prevalence over 2004-2010:
\begin{equation}
\alpha \equiv \displaystyle \sum_i \mbox{Pr}(Z_i=1 \mid \X_i) = \displaystyle\sum_i \frac{\mbox{Pr}(Z_i=1, W_i = 1 \mid \X_i)}{\mbox{Pr}(W_i = 1 \mid Z_i = 1, \X_i)}.
\end{equation}
Because we only obtain measurements on firms who cheated and got caught, the data are only informative about $\Pr(Z_i=1, W_i=1\mid \X)$. Equivalently, for each firm-year we observe $Y_i \equiv Z_iW_i$ instead of $(Z_i, W_i)$, where $Y_i$ indicating whether a firm received an AER (cheated and got caught). Specifically, this is equivalent to the case described in Section \ref{sec:binreg}, with $U_1 = W$ and $U_2 = Z$.

%Note that $\mbox{Pr}(Y_i = 1 \mid \X_i)$ corresponds to the probability that a firm was issued an AAER in a given year, not the probability that its conduct warranted an AAER.  Again, many firms ``deserving" an AAER do not receive one; not all cheaters get caught.  To make this distinction explicit, we introduce two latent variables $Z_i$ and $W_i$ denoting ``cheating" and ``getting caught", respectively. Interest is in estimating the overall prevalence of accounting misconduct in the U.S. economy (between 2004 and 2012), which we define as 
%\begin{equation}
%\alpha = \displaystyle \sum_i \mbox{Pr}(Z_i=1 \mid \X_i) = \displaystyle\sum_i \frac{\mbox{Pr}(Z_i=1, W_i = 1 \mid \X_i)}{\mbox{Pr}(W_i = 1 \mid Z_i = 1, \X_i)}.
%\end{equation}
To cast this in the framework described in Section \ref{Kadane}, denote 
\begin{equation}
\phi(\X) = \mbox{Pr}(Z=1, W = 1 \mid \X) = \mbox{Pr}(Y  = 1 \mid \X); \;\;\; \theta(\X)  = \mbox{Pr}(W = 1 \mid Z = 1, \X).
\end{equation} 
%
Here $\phi(x)$ is simply the distribution of the observed data, and is point identified.  We estimate it using the BART model with default priors, except we set $k=3$.  This choice shrinks $\phi(\X)$ more strongly away from zero or one, which is particularly important in regions of predictor space with very few observations. In particular, it is unrealistic to expect that any company is {\em certain} to both cheat and get caught. The remaining parameter $\theta(x)$ is not identified and an informative prior must be supplied.  

\subsection{Simulated example}\label{sec:ex}
Before turning to the subject-specific prior we developed for our empirical application, it is instructive to consider how our approach performs in a situation where we know what the right answers ought to be. For this purpose we have design a simulated data set emulating the model in \cite{Wang2013}. This will be useful later when comparing our results to those in \cite{Wang2013} on the SEC data.

\subsubsection{A partially observed bivariate probit model}
Inspired by the approach of \cite{Poirier1980}, \cite{Wang2013} proposes a bivariate probit model for the $(W, Z)$ pairs described above.  In this formulation 


\subsection{Surveillance model}
The unidentified function $\theta(\X)$ can be thought of as a ``surveillance" probability; it encodes which attributes invite (discourage) SEC scrutiny, making cheaters more (less) likely to be caught.  Its effect is to inflate the probability of cheating, which is intuitive since the proportion of caught cheaters $\phi(x)$ represents an obvious lower bound on the proportion of actual cheaters.

Our surveillance model takes the form reported in expression (\ref{eq:theta-2}) with  $\epsilon_i \iid \N(0, \sigma^2)$ and using a logit link.  
Some care is required when specifying $h(\X)$. 
%We now describe the specification of $h(\X)$.  
Although BART is invariant to monotone transformations, the linear form of the surveillance model is not so it becomes important to choose transformations of the covariates so that the impact of firm features is plausibly scaled and we can specify reasonable values of $\beta$.  We therefore scale and shift all variables to reside on the unit interval, taking shifted log transformations of the financial times search hits and net income.
%To achieve this, we first  transform selected variables and then we scale and shift all variables to reside on the unit interval.  For our data, only two variables are transformed:  the financial times search hits variable and net income are both log transformed (after adding 1 to avoid taking the logarithm of zero).
%
%Setting the vector of regression coefficients, $\beta$, is where subject matter knowledge can be brought to bear.  Specifically, it allows us to surmise the impact of firm attributes on the probability of getting caught.  
%
We chose to place nonzero coefficients on the (fiscal) year of misconduct, media exposure (as measured by Financial Times search hits), income, cash, and a dummy for qui tam industries. We have specific reasons to expect that these variables are important determinants of the surveillance probability, allowing us to chose informative values for $\beta$.

First, note that the frequency of AAERs is substantially higher in earlier years; see Figure \ref{aaers}. AAERs may be filed retroactively, so the opportunity to discover and report misconduct in a given year increases over time.
%This is likely a simple byproduct of the fact that older cases of misconduct have had a longer time in which to be uncovered.  
%This suggests a negative coefficient on the fiscal year variable, meaning that more recent years are less likely to be spotted (yet).  
Fitting a curve to the data in Figure \ref{aaers} suggests a coefficient $\beta_{fyear} = -2.5$.  Observe that this makes the posterior probability of cheating approximately constant across the years examined, which seems plausible.
\begin{figure}
\begin{center}
\includegraphics[width=3in]{sec-figure/aaer_rate.pdf}
\end{center}
\caption{AAERs appear more common in more distant years, but this is likely because they may be filed retroactively.}\label{aaers}
\end{figure}

Second, it is reasonable to assume that media attention naturally draws SEC scrutiny \citep{miller2006press}.  
%Media darlings such as Apple, Amazon, and Google may be closely monitored because the SEC has a vested interest in making examples of such prominent businesses, should they misbehave.  
The SEC has a vested interest in catching and making examples of any high-profile cheaters.
We set $\beta_{FThits}=2$, implying approximately a six-fold difference in the probability of misconduct being discovered between a company with no media exposure and the company with the highest media exposure. Similarly, we set $\beta_{quitam}=1$, implying approximately a two-fold increase in misconduct being discovered for companies in qui tam industries where employees are incentivized to report misconduct.

These observations constitute the subjective information contained in our first observation model (A).  
To determine the intercept term, consider the following argument: AAERs are quite rare, with an aggregate incidence in our sample of only 0.5\%.  Potentially this is because very few firms exhibit actionable misconduct, but more likely it is because the SEC has limited resources to identify and pursue violations.  Accordingly, one sensible calibration method would be fix the mean probability of discovery across all firms.  Fixing this quantity and the other elements of $\beta$, we may then solve for the intercept $\beta_0$. In the case of model A, fixing the average discovery rate to 30\% gives $\beta_0 = 0$.

After obtaining posterior samples under model A, we observe that cash appears to have a negative impact on the probability of cheating. In contrast, net income appears to have a positive impact on the probability of cheating. We might surmise that these trends are due to unadjusted surveillance probabilities.  For example, one could argue that having large amounts of cash on hand (relative to total assets) provides a measure of ``wiggle room" that makes certain kinds of misconduct harder to discover.  Likewise, firms with high income are more likely to draw SEC attention than firms with smaller income streams.  To compare our results under these narratives, we specify a second surveillance model (B), with $\beta_{cash} = -1.5$ and $\beta_{income} = 2.5$.  Setting the intercept for model B to match the 30\% discovery rate of model A gives $\beta_0 = -0.85$.  Surveillance models  A and B are shown side-by-side in Table \ref{surveillance}.

\begin{table}
\begin{center}
\begin{tabular}{c|cccccc}
&Intercept&Fiscal year &FT.com hits&cash&net income&qui tam\\
\hline 
$\beta_A$ & $\;\;\;0$& $-2.5$&$2$&$0$& $0$& $1$\\ 
$\beta_B$ &$-0.85$&$-2.5$& $2$&$-1.50$&$2.5$&$ 1$\\
\end{tabular}\caption{Regression coefficients defining surveillance models A and B.  They differ in their intercept terms and their cash and net income coefficients.  The intercepts have been adjusted to obtain an average misconduct discovery rate of 30\%}\label{surveillance}
%the media-visibility proxy FT.com hits.  The intercepts have been adjusted to match the overall average probability of being caught, at 30\%.}
\end{center}
\end{table}

\subsubsection{Upper bounding cheating}\label{cparm}
Finally, we introduce an additional parameter $c$ to enforce a stochastic upper bound on the probability of cheating.  Recall that the partial identification in this application is driven by the inequality $\mbox{Pr}(Z = 1 \mid \X) = \frac{\phi(\X)}{\theta(\X)} \leq 1$, which implies $\phi(\X) \leq \theta(\X)$; the left hand side of this latter inequality is identified by the data.  
%If we are willing to stipulate that for any covariate values $\X$ a firm's probability of cheating is strictly less than one, this inequality instead becomes 
Extremely high probabilities of cheating are implausible, motivating us to consider alternative truncations: $\mbox{Pr}(Z = 1 \mid \X) = \frac{\phi(\X)}{\theta(\X)} \leq c$, which implies $\phi(\X)/c \leq \theta(\X)$ for $c \geq \phi(\X)$.  Because $\phi(\X)$ is identified, the data may contradict any particular value of $c$ by violating $c \geq \phi(\X)$ so $c$ is itself partially identified.  We continue our modular prior approach, placing a $\mbox{Beta}\left(10 c_0, 10(1-c_0)\right)$ prior on $c$, which {\em a posteriori} is sampled to obey the truncation implied by $\phi(\X)$.  Intuitively, the prior mean $c_0$ captures prior beliefs about the upper bound on $\mbox{Pr}(Z = 1 \mid \X)$, the probability of cheating for any firm.  

Our surveillance models allow us to include prior information in the form of
%As constructed, our surveillance models allow not only 
subject matter knowledge about the impact of various covariates. %to be incorporated, but also permit
We are also able to include additional subjective prior information about $\sum_i \mbox{Pr}(W_i = 1 \mid Z_i = 1, \X_i)$ --- the overall average probability of a cheating firm getting caught --- via the intercept terms, and $\mbox{max}_i \mbox{Pr}(Z_i = 1 \mid \X_i)$ --- an upper probability on any firm cheating --- via the prior on $c$. It would be difficult to acheive all these simultaneously without using the modular prior approach, which also facilitated the sensitivity analysis described below and a number of other iterations over candidate surveillance models that we do not have space to describe here.



\subsection{Results}
We conduct a sensitivity analysis by varying the parameters $\sigma$ and $c$ for both model coefficients $\beta_A$ and $\beta_B$ above.  Specifically, we consider two settings of each ($\sigma \in \lbrace 0.25,0.5 \rbrace$ and $c \in \lbrace 0.4,0.8 \rbrace$) for a total of eight candidate models.  We study the impact these choices have on both $\mbox{Pr}(Z=1 \mid \X)$ as a function of individual predictor variables, and also on the overall misconduct prevalence $\alpha$.

Figure \ref{SICboxplot} shows the posterior distribution of the adjusted cheating prevalence under the different models. As can be seen in the left-hand panel, increasing $\sigma$ or $c$ alone has little effect on the overall adjusted cheating prevalence. These two parameters control different aspects of the surveillance uncertainty: a high $c$ implies that any probability of cheating is plausible, whereas a high $\sigma$ allows large deviations from the specified surveillance model logistic term.  Note that with the range of $c$ and $\sigma$ chosen, neither surveillance model yields overall prevalence of misconduct greater than 15\%.

The right-hand panel of Figure \ref{SICboxplot} shows the posterior prevalence for each different SIC code under the two priors, fixing $(\sigma=0.25, c = 0.4)$. Under both priors, SIC category D, representing ``electricity, gas, steam and air conditioning supply'', shows much lower cheating prevalence than categories (B,E,H), which correspond to ``mining and quarrying'', ``water supply, sewerage, waste management and remediation activities'', and ``transportation and storage'' respectively. 
\begin{figure}
\begin{center}
\includegraphics[width=\textwidth]{sec-figure/boxplots.pdf}\\
\includegraphics[width=\textwidth]{sec-figure/SICboxplot.pdf}
\end{center}
\caption{Top panel: posterior cheating prevalence, white corresponding to the raw (unadjusted) prevalence, pink to prior A and blue to prior B. The four boxplots within each prior correspond to the following combinations for $c$ and $\sigma$ (from left to right): $(\sigma=0.25,c = 0.4),\;(\sigma=0.25, c = 0.8 ),\;(\sigma=0.5, c=0.4),\;(\sigma=0.5, c= 0.8)$. Bottom panel: Posterior cheating prevalence in companies within each SIC code, pink corresponding to prior A and blue to prior B for $(\sigma=0.25,c=0.4)$.  }\label{SICboxplot}
\end{figure}

Because BART is nonlinear, summary plots of the impact of individual covariates are challenging to visualize, even if the surveillance model is relative simple, such as our linear logistic specification.  It is instructive, therefore, to examine the implied probability of cheating as one varies individual covariates, for a given firm.  That is, how does $\mbox{Pr}(Z=1 \mid \X)$ change as a function of $x_j$ while holding $x_{-j}$ fixed?

To demonstrate this approach, we focus on a specific firm, ConAgra Foods of Omaha, Nebraska (simply because it yields illustrative plots).  Figure \ref{VaryPriorVarySC} shows $\mbox{Pr}(Z=1 \mid \X)$, varying media attention, cash, and net income under priors A and B and for various combinations of $c$ and $\sigma$. As expected, the surveillance model coefficients on cash and net income reverse the associated slope of the probability of cheating.  High values of both $\sigma$ and $c$ results in posterior credible intervals of up to 40\% probability of cheating for some values of net income. 

We have reported here only a small number of the possible variations one would presumably want to investigate; we make no claims that models A and B are ideal or even necessarily good or realistic models.  Rather, our sensitivity analysis demonstrates a range of possible comparisons that one might undertake when investigating how various assumptions interact with the data via the identified portion of the model.  

An important upshot of our analysis is that the surveillance model intercept terms---which govern the  average probability of misconduct discovery (getting caught) across firm---and the parameter $c$--- which defines the upper bound $\mbox{Pr}(Z_i =1 \mid \X_i) \leq c$ for all $i$ --- play dominant roles in determining the inferred overall prevalence of misconduct.  For our choices of 30\% misconduct discovery probability and $c = 0.4$ or $c=0.8$, we find that no more than 15\% of firms engage in accounting misconduct.  


\begin{figure}
\begin{center}
\includegraphics{sec-figure/priorAB.pdf}
\end{center}
\caption{$\mbox{Pr}(Z=1 \mid \X)$ varying $x_j$ while holding $x_{-j}$ fixed (at the values of ConAgra Foods) under two surveillance models A (pink) and B (blue). Lines depict the median and shaded areas depict 90\% credibility intervals. Each row represents a different covariate; the three columns correspond to the following $(c, \sigma)$ combinations (from left to right): $(c=0.4,\sigma=0.25),\;(c=0.8,\sigma=0.25),\;(c=0.8,\sigma=0.5)$. }\label{VaryPriorVarySC}
\end{figure}
